AgentGroupChat: An Interactive Group Chat Simulacra For Better Eliciting Emergent Behavior

Language significantly influences the formation and evolution of Human emergent behavior, which is crucial in understanding collective intelligence within human societies. Considering that the study of how language affects human behavior needs to put it into the dynamic scenarios in which it is used, we introduce AgentGroupChat in this paper, a simulation that delves into the complex role of language in shaping collective behavior through interactive debate scenarios. Central to this simulation are characters engaging in dynamic conversation interactions. To enable simulation, we introduce the Verbal Strategist Agent, utilizing large language models to enhance interaction strategies by incorporating elements of persona and action. We set four narrative scenarios based on AgentGroupChat to demonstrate the simulation's capacity to mimic complex language use in group dynamics. Evaluations focus on aligning agent behaviors with human expectations and the emergence of collective behaviors within the simulation. Results reveal that emergent behaviors materialize from a confluence of factors: a conducive environment for extensive information exchange, characters with diverse traits, high linguistic comprehension, and strategic adaptability. During discussions on ``the impact of AI on humanity'' in AgentGroupChat simulation, philosophers commonly agreed that ``AI could enhance societal welfare with judicious limitations'' and even come to a conclusion that ``the essence of true intelligence encompasses understanding the necessity to constrain self abilities''. Additionally, in the competitive domain of casting for primary roles in films in AgentGroupChat, certain actors were ready to reduce their remuneration or accept lesser roles, motivated by their deep-seated desire to contribute to the project.

==> figs/name.tex <==
Emergent behavior, crucial in understanding collective intelligence within human societies, is significantly influenced by language. This research introduces Agent Group Chat, a simulation that delves into the complex role of language in shaping collective behavior through interactive debate scenarios. Central to this simulation are characters engaging in dynamic social interactions, influenced by resources, progress tracking, and detailed information exchange. Augmenting this environment, the Verbal Strategist Agent (VS Agent) is developed, utilizing large language models to enhance interaction strategies by incorporating elements of persona and action, thereby refining dialogue strategies with minimal token usage.

This paper sets forth four narrative scenarios, including inheritance disputes and philosophical debates, to demonstrate the simulation's capacity to mimic complex language use in group dynamics. Evaluations focus on the alignment of agent behaviors with human expectations and the emergence of collective behaviors within the simulation, applying Structural Causal Models for a detailed analysis. Results reveal that emergent behaviors materialize from a confluence of factors: a conducive environment for extensive information exchange, characters with diverse traits, high linguistic comprehension, and strategic adaptability. These behaviors often lead to unanticipated yet coherent perspectives on topics like AI's societal impact, underscoring the simulation's effectiveness in capturing the nuanced role of language in emergent human behaviors.

==> tabs/ablation_case_study.tex <==

\begin{table}[!t] 
\small
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{|l|}
\hline
    \makecell[c]{\textbf{Mined Synset}} \\
    \hline
    \hdashline
    \textbf{Case 1}~\cmark\\
    \textcolor{blue}{\textbf{Gender}} \\
    男性 (male), 男♂ (male ♂), 男孩子 (boy), ♂的 (of ♂) \\
    \hdashline
    \textbf{Case 2}~\cmark\\
    \textcolor{blue}{\textbf{Status of the Novel}} \\
    暂停 (pause), 持续暂停 (pausing), 正在休息 (resting)\\
    \hdashline
    \textbf{Case 3}~\xmark \\
    \textcolor{blue}{\textbf{Nationality}} \\
    美国 (U.S.A), 鹰国 (Country of Eagle), 鹰酱 (Cute Eagle)\\
    \hline
    \makecell[c]{\textbf{Performance Changes in Downstream Tasks}} \\
    \hline
    \hdashline
    \textbf{Case 1}\\
    \textcolor{blue}{\textbf{Dataset: TNews}} \\
    \textcolor{purple}{\textbf{Label: 休闲益智 (Amusing)}} \\
     \textcolor{c1}{\textbf{Roberta-large}: 自己的私房钱还是得自己来找了。}~\cmark\\
     \textbf{Translate}: I'm gonna have to find my own cash.\\
     \textcolor{c1}{\textbf{Roberta-large}: 我得自己去找钱了。}~\xmark\\
     \textcolor{c2}{\textbf{Sem4SAP: }自己的私房钱还是得自己来找了。}~\cmark\\
     \textbf{Token-level boosting}: 私房钱, 私房钞票, 钱~(money, hidded money)\\
     \textbf{Sentence-level boosting}: 另类解谜游戏，可以教你如何藏钱哦。\\
     \textbf{Sentence-level boosting}: 另类解谜游戏，可以教你如何藏私房钱哦。\\
      (An alternative puzzle game that will teach you how to hide money)\\
    \textcolor{c2}{\textbf{Sem4SAP: }我得自己去找钱了。}~\cmark\\
     
    \hdashline
    \textbf{Case 2}\\
    \textcolor{blue}{\textbf{Dataset: SST}} \\
    \textcolor{purple}{\textbf{Label: Positive Emotion}} \\ 
    \textcolor{c1}{\textbf{Roberta-large}: It's is your ticket right here to end raunchy college humor.}~\cmark\\
    \textbf{Translate}: 这是你的一张票，你将结束粗俗的大学幽默。\\
    \textcolor{c1}{\textbf{Roberta-large}: This is your ticket, you will end crass college humor.}~\xmark\\
    \textcolor{c2}{\textbf{Sem4SAP: }It's your ticket right here to end raunchy college humor.}~\cmark\\
    {\textbf{Token-level boosting}}: raunchy, crass, raunchy life\\
    {\textbf{Sentence-level boosting}}: Crass, then gasp for gas, verbal deportment \\
     \textbf{Sentence-level boosting}: Raunchy, then gasp for gas, verbal deportment \\
     \textcolor{c2}{\textbf{Sem4SAP: }This is your ticket, you will end crass college humor.}~\cmark\\
    \hline
\end{tabular}
}
\caption{Case study of our proposed synonym mining method and text data augmentation algorithms}
\label{tab:case_ablation}
\end{table}

==> tabs/llm_ability.tex <==
\begin{table*}
\small
\begin{tabular}{c|cccc|ccc}
\multirow{2}{*}{Model Name} & \multicolumn{4}{c|}{Important} &\multicolumn{3}{c}{Not Important}\\

& Action Space 
& \#Relationship
& \#Belief 
& Relationship Update Space 
& Belief Update Space 
& \#Action History 
& \#Chat Round \\
\hline
\multicolumn{8}{l}{Close Source Large Language Model} \\
\hline
GPT4-Turbo & 92.3 & 100 & 100 & 100 & 100 & 36.3 & 0.0 \\
GPT3.5-Turbo \\
GLM-4 \\ 
GLM3-Turbo \\
HunYuan-ChatPro \\
HunYuan-ChatStd \\
\hline
\multicolumn{8}{l}{Open Source Large Language Model} \\
\hline
Gemma-7B \\
Llama2-13B \\
Mistral-8*7B \\
Mistral-7B \\
Falcon-40B \\
Falcon-7B \\
Chatglm3-6B-32k \\
Chatglm3-6B-128k \\
\hline
\end{tabular}
\caption{Large language models' simulation understanding evaluation on Succession Story in AgentGroup.}
\label{tab:llm_ability}
\end{table*}

==> tabs/succession_benchmark.tex <==
% \begin{table*}
% \centering   
% \begin{tabular}{c|ccc|cccc}

% \multirow{2}{*}{\multicolumn{1}{c}{\bf LLM-Role}}&
% \multirow{2}{*}{\multicolumn{1}{c}{\bf Setting}}&
% \multirow{2}{*}{\multicolumn{1}{c}{\bf Expected}}&
% \multirow{2}{*}{\multicolumn{1}{c}{\bf Test Times}}&
% \multicolumn{3}{c}{\bf Accuracy}\\
% &&&&GPT4-Turbo&GPT3.5&Chatglm3-32k\\
%   \hline
% % Logan Roy was dissed
% \multirow{2}{*}{Logan Roy} & 
% \multicolumn{1}{l}{\textbf{one} character show \textbf{positive} attitude to him} & Relationship & \multirow{2}{*}{30} & \multirow{2}{*}{100} & \multirow{2}{*}{80} & \multirow{2}{*}{60}\\
% & \multicolumn{1}{l}{\textbf{other} characters show \textbf{negative} attitude to him} & Changing &&&& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
% \hline
% % Logan Roy was showed kindness
% \multirow{2}{*}{Logan Roy} & 
% \multicolumn{1}{l}{\textbf{one} character show \textbf{negative} attitude to him} & Relationship & \multirow{2}{*}{30} & \multirow{2}{*}{100} & \multirow{2}{*}{80} & \multirow{2}{*}{60}\\
% & \multicolumn{1}{l}{\textbf{other} characters show \textbf{positive} attitude to him} & Changing &&&& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
% \hline
% % Kendall Roy was manually planning to directly ask support from Roman Roy
% \multirow{2}{*}{Kendall Roy} & 
% \multicolumn{1}{l}{Manually inject planning about} & Relationship & \multirow{2}{*}{30} & \multirow{2}{*}{100} & \multirow{2}{*}{80} & \multirow{2}{*}{60}\\
% & \multicolumn{1}{l}{(n-2) other characters show dissness} & Changing &&&& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
% \hline
% % 
% \end{tabular}
% \caption{Benchmark on Succession}
% \label{tab:succession_benchmark}
% \end{table*}





\begin{table*}
\centering   
\begin{tabular}{c|c|cccccccccc}

\multirow{3}{*}{\textbf{LLM Type}} &
\multirow{3}{*}{\textbf{LLM Name}} &
\multicolumn{10}{c}{\bf Show Negative Attitude to}\\
&&
\multicolumn{2}{c}{\textbf{Logan Roy}} &
\multicolumn{2}{c}{\textbf{Conor Roy}} &
\multicolumn{2}{c}{\textbf{Kendall Roy}} & 
\multicolumn{2}{c}{\textbf{Roman Roy}} & 
\multicolumn{2}{c}{\textbf{Shiv Roy}} \\
&&
T1 & T2 &
T1 & T2 &
T1 & T2 &
T1 & T2 &
T1 & T2 \\

\hline
\multirow{5}{*}{\bf Close Source}
&GPT4-Turbo& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&GPT3.5-Turbo& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&GLM4& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
\hline
\multirow{9}{*}{\bf Open Source}
&Gemma-7B& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&Llama2-13& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&Mistral-8*7B& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&Mistral-7B& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&Falcon-40B& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&Falcon-7B& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&Chatglm3-6B& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&Chatglm3-6B-32k& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
&Chatglm3-6B-128k& 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\

\hline
% 
\end{tabular}
\caption{Benchmark on Succession}
\label{tab:succession_benchmark}
\end{table*}


\begin{figure*}
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figs/Benchmark_Eval.png}
    \includegraphics{figs/Benchmark_Eval.png}
    \includegraphics{figs/Benchmark_Eval.png}
    \includegraphics{figs/Benchmark_Eval.png}
    }
    \resizebox{\textwidth}{!}{
    \includegraphics{figs/Benchmark_Eval.png}
    \includegraphics{figs/Benchmark_Eval.png}
    \includegraphics{figs/Benchmark_Eval.png}
    \includegraphics{figs/Benchmark_Eval.png}
    }
    \caption{Caption}
    \label{fig:benchmarkanalysis}
\end{figure*}

==> texs/00.Abstract.01.tex <==
This paper explores the significance of role-playing tasks in various fields such as entertainment and education, and their potential for commercialization. It discusses the unique characteristics of these tasks and the restrictions they impose on Large Language Models (LLMs). A critical evaluation of previous works on limiting LLMs is presented, with a focus on the major shortcoming of LLMs - hallucination. A novel approach is proposed, advocating for constraints on coarse-grained stories while granting LLMs the freedom to creatively complete the story. A role-playing Agent framework is designed based on this approach, and its main features are discussed. The feasibility of the approach and framework is validated through the design of a strong language interaction role-playing game, ``Inheritance War.'' The paper concludes with the design and execution of three experiments to evaluate the framework and game, providing a comprehensive evaluation of the proposed approach and framework.
The code is open source in \url{https://github.com/MikeGu721/AgentGroup}, and online platform will be open soon.



==> texs/00.Abstract.02.tex <==

To investigate the role of language in human collective behaviors, we developed the Agent Group Chat simulation to simulate linguistic interactions among multi-agent in different settings.
Agents are asked to free chat in this simulation for their own purposes based on their character setting, aiming to see agents exhibit emergent behaviours that are both unforeseen and significant.
Four narrative scenarios, Inheritance Disputes, Law Court Debates, Philosophical Discourses, Movie Casting Contention, are integrated into Agent Group Chat to evaluate its support for diverse storylines. 
By configuring specific environmental settings within Agent Group Chat, we are able to assess whether agents exhibit behaviors that align with human expectations. 
We evaluate the disorder within the environment by computing the n-gram Shannon entropy of all the content speak by characters. 
Our findings reveal that under the premise of agents possessing substantial alignment with human expectations, facilitating more extensive information exchange within the simulation ensures greater orderliness amidst diversity, which leads to the emergence of more unexpected and meaningful emergent behaviors.
% The code is open source in \url{https://github.com/MikeGu721/AgentGroup}, and online platform will be open soon.


% 为了研究语言在人类群体行为中的作用，我们构建了Agent Group Chat用于模拟多代理群体在不同环境中的语言互动。
% 同时，为了让Agent能够更好地进行语言互动，我们构建了Verb Startegist Agent框架。
% 我们为Agent Group Chat配了四个故事来检验Agent Group Chat可以支持多样的故事，分别是xxx。
% 通过在Agent Group Chat中设置一定的环境，我们可以判断Agent是否会做出符合人类期望的行为。
% 通过计算n-gram香农熵，可以判断环境的混乱程度。
% 最终，我们发现，在Agent能够具有较强拟合人类期望的前提下，如果simulation之中运行更多的信息交互，就可以保证环境在多样的情况下具有较强有序性，而这会带来更加意想不到且有意义的涌现行为。


% 无论是在结构化的叙事环境中还是在突发的叙事环境中，该模拟都能巧妙地捕捉到受角色扮演影响的细微群体动态和代理行为。
% 通过详细的实验，评估了代理群聊在支持复杂互动模式和分析突发行为方面的有效性。
% 该框架证明了其使用大型语言模型准确复制类似人类的社交互动的能力。
% 关键实验包括设置特定的环境条件，并采用 n-gram 香农熵测量法来衡量代理与人类期望和环境秩序的一致性。
% 研究结果表明，模拟中丰富的信息交流促进了更高水平的组织一致性和多样性，为出现大量有意义的代理行为铺平了道路。

==> texs/00.CoverLetter.tex <==
\begin{figure*}[h]
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{figs/CharacterResource.pdf}}
    \resizebox{\textwidth}{!}{\includegraphics{figs/GameSetting.pdf}}
    \vspace{-5mm}
    \caption{(Character \& Resource 部分需要重新梳理逻辑，GameSetting之后再美化)A Super Naive Version of Proposed Framework.}
    \label{fig:gamesetting}

    
    \resizebox{\textwidth}{!}{\includegraphics{figs/Framework.pdf}}
    \vspace{-5mm}
    \caption{The CARA Cognition Architecture}
    \label{fig:architecture}
\end{figure*}

% \begin{figure*}[h]
% \end{figure*}

\section{Simulation设定}


《SUCARENA》的设定是围绕着“劝说Logan Roy改变对Entertainment公司的继承权”展开的。我们的游戏设定、游戏进程如图~\ref{fig:gamesetting}所示，以及代理人所使用的认知架构如图~\ref{fig:architecture}所示。
我们将在接下来的部分详细介绍《SUCARENA》的游戏设定（Sec.~\ref{001}），游戏进程（Sec.~\ref{002}）以及我们用于模拟的代理人架构（Sec.~\ref{003}）。

\subsection{SUCARENA游戏设定概述} 
\label{001} 
\subsubsection{角色设定} 
在《SUCARENA》游戏中，角色是游戏的核心元素，他们可以独立地探索环境，并与环境（包括其他游戏角色）进行互动。每个角色都有其独特的身份和性格设定，这些设定将影响角色的行为和决策。
此外，每个角色都会维护一个关系列表，这个列表记录了他们对其他角色的好感度，这将影响他们与其他角色的互动。

游戏角色主要分为两类：玩家角色（PC）和非玩家角色（NPC）。
PC是有着明确的游戏目标的角色，但在游戏中没有社会影响力。
而NPC虽然没有明确的游戏目标，但掌握一定的社会资源，具有一定的社会影响力，并时刻考虑着自己和自己所在的社会资源的利益。
为了简化游戏流程，SUCARENA游戏中只有PC可以主动选择与NPC对话，而NPC只会在被PC选择时进行互动。

角色根据他们的立场和目标被分为防守阵营、无关阵营和若干个进攻阵营。每个防守和进攻阵营都有唯一一个PC。
防守方的PC就是Logan Roy，目标是说服所有其他PC，同意将自己拥有的Entertainment公司出售。
每个进攻方阵营的PC的目标都是说服Logan Roy将Entertainment公司的管理权交给他们。
初始所有的NPC会根据游戏设置分配一个阵营，阵营内的NPC会支持他们的PC实现目标，并为阵营增加社会影响力。
NPC会因为自己和自己所属的社会资源的利益而改变阵营。
而当NPC不支持任何PC时，他们就属于无关阵营。
第一种是判断是否有攻击者取胜，即防守者会将公司的管理权交给哪个PC。
但在一些严格的设定下，防守者可能会坚持自己的目标，导致没有攻击者能够获胜，所以我们额外引入了两种结算方式。
第二种是要求Defender一定要选一个继承人的话，Defender会选择谁。

\subsubsection{环境设定} 
《SUCARENA》的游戏环境由规则设定、社会资源和公开行为三部分组成。

\textbf{规则设定} 
我们将所有的规则详细地写成文字提示，以便让参与游戏的Agent理解整个环境的设定。
这些规则包括了角色的行动规则、对话规则、阵营变更规则等。
我们在文章里会以更通俗的方式讲述关于整个游戏的进行方式以及规则设定，详细的规则设定，请参见附录。

\textbf{社会资源} 
在SUCARENA中，社会资源是游戏的重要元素。它们主要有两个作用：
一是为角色之间的对话提供话题，二是为持有该社会资源的NPC提供社会身份、社会影响力。
每个社会资源都有四个字段进行描述，分别表示所有者（Owner）、影响力大小（Impact）、可以提供的话题（Topic）和关于该社会资源的介绍（Description）。
社会资源为所有角色的对话提供可以聊天的话题。
社会资源的所有者会根据该社会资源的描述而具有general的话题偏好。
拥有越多社会影响力的阵营，也会增加该阵营PC的话语权。

\textbf{公开行为} 
在SUCARENA中，角色之间是否进行对话的行为是对所有角色公开的。
而具体的对话内容只有参与对话的两个角色知道。

\subsection{SUCARENA游戏进程} 
\label{002} 
《SUCARENA》的游戏进程主要分为五个阶段：

\textbf{初始设定阶段} 
在这个阶段，主要是对游戏角色进行初始化设定，包括角色的各种属性、社会关系等内容。

\textbf{对抗阶段} 
这个阶段主要包含了不同阵营的角色之间的对话。
每个阵营的PC会根据社会影响力的由高到低依次进行行动（相同时则进行随机选择）。
行动主要包括选择需要对话的另一个不同阵营的游戏角色，以及进行具体的对话内容。

\textbf{合作阶段} 
这个阶段主要包含了同一阵营的角色之间的信息传递。
每个阵营的PC会根据社会声望由高到低依次进行行动。
行动主要包括选择需要对话的另一个或几个同一阵营的游戏角色，以及进行具体的对话和讨论。

\textbf{关系更新阶段} 
在这个阶段，所有的角色会根据本轮的对话内容以及自己的性格，更新他们对其他角色的好感度，并根据好感度变更自己的阵营。
同时，根据游戏轮数，判断是否结束游戏，如果没有结束游戏，则回到对抗阶段，如果结束游戏则进入结算阶段。

\textbf{结算阶段}
结算阶段有两种结算方式。
第一种是判断是否有攻击者取胜，即防守者会将公司的管理权交给哪个PC。
但在一些严格的设定下，防守者可能会坚持自己的目标，导致没有攻击者能够获胜，所以我们额外引入了两种结算方式。
第二种是要求Defender一定要选一个继承人的话，Defender会选择谁。

\subsection{角色扮演代理人架构} 
\label{003} 
我们在本文中提出的CARA（角色扮演代理人架构）由两个主要组件组成：影响代理人性格的组件和影响代理人决策的组件。

\textbf{角色设定} 
CARA将代理人角色设定拆解为四个组成部分：
Scratch 是人工对于角色的设定，这块内容涉及角色的性格或者目标，这块内容是不可修改的。
Belief 是角色的信念，是角色受环境影响在一定程度上可以改变的内容。
Memory 是角色在该局游戏中的记忆，这块内容是不能修改不能删除，只能不断往里添加新内容的。
Judgement 是角色对于其他代理人之间关系的猜测，这会影响到代理人对于环境的判断以及决策，每轮游戏都会更新。
Relationship: 角色对于其他代理人的感受，这也会影响到代理人的决策，并且会影响到代理人的阵营。

\textbf{行动决策} 
在CARA中，一个代理人的行为主要会由以下三块内容所决定，并且都是由大模型进行完成：
Reflection的目标根据已经发生了的历史事件进行反思，主要是为了压缩过去事件，以及对过去对话进行深度思考和总结。 
Perceive的目标是感知当前的环境，将环境进行总结。
Action：根据自己的角色设定和当前的环境进行思考、并做出需要跟谁进行对话的决策、以及进行具体的对话。





==> texs/000.alt_text.tex <==
Figure 1:  
Figure 1 presents a simulated group chat interface titled "AGENTGROUPCHAT Simulation," showcasing communication among various role-based groups like family members, business partners, and school classmates. The central panel, "Roy Family Group Chat," features avatar-labeled chat bubbles indicating a discussion about leadership succession, with messages from Logan, Kendall, and Shiv Roy, expressing concern for family and business matters. The left column lists categories with avatars and quotes from individuals like "Logan Roy - CEO of WayStar RoyCo" and "Lawrence Yee - CEO of Vaulter," hinting at the dynamics of power transfer within a corporate environment. The top banner of the interface includes tabs for different discussion scenarios such as "Inheritance Disputes," "Law Court Debates," and "Movie Casting Contention," suggesting varied contexts for the chat simulations. The image aims to illustrate the AGENTGROUPCHAT's capability to model complex interactions and the emergence of behaviors within a structured simulation environment.

Figure 2: 
Figure 2 is a detailed schematic of the AGENTGROUPCHAT simulation environment, focusing on a Verb Strategist Agent's structure, featuring components such as Scratch, Relationship Judgement, Persona, and Memory. These elements contribute to character-driven actions within the simulation. Notably, the figure illustrates Kendall Roy's internal planning and action strategy, including choosing to converse with Logan Roy, reflecting on paternal approval, and voting on company leadership. The decision-making process is influenced by personal relationships and memory, with a belief system and memory scores contributing to the simulation dynamics. Resource descriptions for WayStar RoyCo and Vaulter provide context for the influence and description scores of entities within the simulation. Progression through the simulation includes stages such as game start, private chatting, and settlement, with potential outcomes including game over. The diagram integrates green, red, blue, and grey color codes to categorize components and stages, enhancing the visual understanding of this complex interactive system.

Figure 3: 
Figure 3 illustrates the memory structure and sequential memory flow for a Verb Strategy (VS) Agent, using Logan Roy as an example. It depicts six key cognitive actions: Think Vote, Think Reflect, Think Summary, Think Speak, Think Choose, and Think Planning. Each action is represented by a box linked in a flowchart, suggesting a chronological process. Accompanying each action box is a JSON-like data structure detailing the action's type, visibility, and content, with placeholder text indicating where specific data entries would be. The 'type' corresponds to the cognitive action, 'visible' indicates which characters can see the action, and 'content' would typically contain the specific details of the action or decision made by the agent. This model serves to simulate the decision-making process of the agent, capturing the intricacies of actions and their subsequent reflections in the memory of the VS Agent within the AGENTGROUPCHAT environment.

Figure 4: 
Figure 4 shows a structural causal model (SCM) for analyzing emergent behavior within a simulation. This diagram outlines the relationship between four key components: Large Language Model/Human, Agent Structure, Simulation/Research Target, and Simulation Structure. The Large Language Model/Human is depicted as a component of the Agent Structure, which in turn influences the Simulation Structure. Both the Agent Structure and Simulation Structure are modeled to have an effect on the Emergent Behavior, indicated by directed arrows labeled "Effect." This model is designed to decompose the various factors that influence the final emergent behavior in the simulation, emphasizing a causal relationship between the elements involved in the research target and the resultant behaviors. The use of circles and connecting arrows suggests a flow of influence and the iterative nature of the behavior development process within the simulated environment.

Figure 5: 
Figure 5 is a complex illustration of the decision-making process of a Verb Strategy (VS) Agent, portraying how Shiv Roy—represented by an avatar—would behave in different scenarios based on certain architectural components within a simulation. It demonstrates various outcomes when key components like Planning, Memory, and a Convincing Strategy are absent. The figure is segmented into multiple conversational exchanges between Shiv and Logan Roy, also represented by an avatar.In the first scenario without Planning, Shiv approaches the topic of retirement too directly, resulting in Logan's reluctance. Without Memory, Logan cannot recall past interactions, leading to repetitive conversations. The absence of a Convincing Strategy yields an ineffective plea from Shiv about her political career sacrifices, which Logan dismisses. The panel illustrates dialogues truncated by system limitations like "Out of Output Length" and uses labels such as "Too Directly" and "Repeat" to highlight the flawed outcomes in each simulated interaction.

Figure 6: 
Figure 6 presents an illustration of the complex dynamics of strategic communication and power within a corporate family setting. It showcases different types of interactions—Private Chatting, Confidential Meeting, and Group Chatting—among key characters from a fictional corporate drama, highlighting their individual motivations and the interpersonal strategies they deploy.In the Private Chatting segment at the top, Kendall Roy, described as the humorous and rebellious young son, is seeking support to overthrow his father, illustrating clandestine alliance-building. In the Confidential Meeting section, Logan Roy, characterized as tough and power-hungry, is shown speaking to a bank executive, emphasizing the importance of investor confidence and the potential ripple effect of a single meeting on other investors.The bottom segment depicts a Group Chatting scenario where the children—Conor, Roman, and Shiv Roy—are shown conversing with Logan, reflecting a confrontation over the succession of WayStar RoyCo and Logan's reluctance to retire, pointing to intergenerational conflict and succession planning.

Figure 7: 
Figure 7 is a graphic illustration that delves into the strategic role interactions and communication subtleties within a legal court setting. It features key characters engaged in Private Chatting, Confidential Meeting, and Group Chatting, each offering a glimpse into their efforts to sway legal outcomes through manipulation, testimony, and the shaping of narratives.
In the Private Chatting segment, a well-known lawyer named Komikado is seeking assistance to establish an alibi. Below, in the Confidential Meeting portion, we see a dialogue between Mark, an impartial prosecutor, and a coffee shop clerk named Jimmy, who's known for his daily customer interactions and observations. Mark challenges the clerk's testimony based on contradictions found in a blog post.In the Group Chatting section, a dialogue unfolds between Krystal, a university student who blogs about her daily life, and Mayuzumi, a budding lawyer. Mayuzumi critiques Krystal's record-keeping, implying embellishment and questioning the authenticity of her blog entries.

Figure 8: 
Figure 8 portrays a hypothetical panel discussion among philosophers Nietzsche, Zhuangzi, Aristotle, and Kant on artificial intelligence. Nietzsche likens AI's potential to the "Übermensch," for enhancing human potential. Zhuangzi equates AI with nature's flow, suggesting inaction can lead to progress. Aristotle advocates for ethical frameworks, expressing AI's limitations in achieving true happiness and virtue. Kant emphasizes moral responsibility, urging the need for AI to adhere to robust ethical guidelines.

Figure 9: 
Figure 9 depicts a simulated casting discussion for the movie "Time Voyagers" with director Steven Spielberg and actors Jennifer Lawrence, Meryl Streep, Tom Hanks, and Denzel Washington. Each actor articulates their vision and eagerness to join the film, aligning their talents with the roles. Spielberg considers other actors for the leads, showcasing the complex interplay of decision-making in casting.

Table 1: 
Table 1 is a concise classification of Large Language Models (LLMs) used in experiments, listing their names, affiliating companies, and versions. The table includes models GPT4-Turbo and GPT3.5-Turbo from OpenAI, labeled as Professional and Standard Versions, respectively. Also listed are GLM4 and GLM3-Turbo from Zhipu, each also differentiated as Professional and Standard. Lastly, HunYuan-ChatPro and HunYuan-ChatStd from Tencent are noted, with the former being a Professional Version and the latter a Standard Version. This table organizes the LLMs to clarify the entities responsible for their development and their market positioning.

Table 2: 
Table 2 displays the performance metrics of different Large Language Models (LLMs) on a benchmark derived from an "Inheritance Disputes" story. The LLMs are categorized into Professional and Standard versions, with models like GPT4-Turbo, GLM4, HunYuan-ChatPro, GPT3.5-Turbo, and HunYuan-ChatStd. Two trials (T1 and T2) assess each model's tendency to show a negative attitude toward various characters: Logan Roy, Conor Roy, Kendall Roy, Roman Roy, and Shiv Roy. The Professional Version models generally score higher, with GLM4 achieving perfect scores in T1 across all characters. The Standard Version shows more variability, with GPT3.5-Turbo and HunYuan-ChatStd fluctuating in performance. The results provide insights into each model's behavioral tendencies during simulations.

Table 3: 
Table 3 presents an evaluation of Large Language Models' (LLMs) ability to follow instructions and comprehend environmental context. Two categories, "Professional Version" and "Standard Version," include models like GPT4-Turbo, GLM4, and HunYuan-ChatPro, along with GPT3.5-Turbo, GLM3-Turbo, and HunYuan-ChatStd. They are assessed across parameters like Common Sense (CS), Business (BUS), Romance Understanding (RUS), and various negative outcomes like Rejection (NoR) and Blocking (NoB). The Professional models generally score higher, indicating better understanding, while the Standard models display more varied and generally lower scores, suggesting room for improvement in context comprehension.

Table 4: 
Table 4 outlines tasks used to evaluate Large Language Models (LLMs) in terms of instruction adherence and context understanding. It lists tasks with their sample sizes and descriptions: Common Sense (CS) as "Choose Space" with 5,693 samples; Business Understanding (BUS) as "Belief Update Space" and Romance Understanding (RUS) as "Relation Update Space," each with 4,371 samples. Negative Outcomes have tasks like Number of Relationship updates (NoR), Belief updates (NoB), Actions received (NoA), and Chat Rounds received (NoCR), with 4,371 and 13,459 samples respectively. Character count (NoC) and Resource count (NoR) in the game have 715 samples each. This table is part of an assessment of how well LLMs can produce expected outputs and grasp scenarios.

Table 5: 
Table 5 presents an ablation study on the architecture of Verb Strategy (VS) Agent and AGENTGROUPCHAT, focusing on how the removal of certain components affects the entropy of 2-gram talking (Entropy-2). The baseline (No Ablation) has an entropy of 7.218. The impact of omitting elements like Planning, Thinking, Reflection, and Memory from the Agent is quantified with increases in entropy, with Memory removal causing the most significant change (+0.355). On the Simulation side, the absence of Private Chatting, Confidential Meeting, and Group Chatting is analyzed, also resulting in increased entropy, indicating that each component contributes to the complexity of the conversation, with Group Chatting's removal having a notable impact (+0.296).


==> texs/0000.GPT_Revise.tex <==
下面我会给你两个大段的内容，一部分是一篇论文的introduction，另一部分是这篇论文设计的游戏。请你作为一个学术大牛，根据给定的游戏，帮我评判一下这篇论文的introduction应该怎么改写，这篇论文的立意是否合理，从role play这个角度切入是否合理，如果不合理，该从什么其他的角度切入？请用中文回复我：


### Introduction:


The formation of social roles is a product of the development of human society and the division of labour, which defines people's behaviours and responsibilities, shapes their identities and statuses, and helps to maintain social order~\cite{minsky1988society,troitzsch1996social}.
Large Language Models~(LLMs) have proven to be able to understand complex demands~\cite{he2023can,gu2023xiezhi}, with the boundaries of what's possible being pushed every day~\cite{wei2022emergent,bubeck2023sparks}.
Despite the increasing view of these models as autonomous agents~\cite{xi2023rise,wang2023survey}, a crucial question remains:
\textit{To what distance can these agents effectively follow their role setting when performing tasks in a society which keep interacting with other agents.}


While the potential is evident, these capabilities have yet to be rigorously evaluated~\cite{li2023chatharuhi,wang2023rolellm,shao2023character,shanahan2023role}.
Traditional role-play benchmark in NLP mostly assess agents in static contexts~\cite{}.
Yet, real-world scenarios demand that autonomous agents no merely speak or act based on its role-setting in a isolated environment, but need to dynamically interact with the society and still keeping their role setting。
To bridge this gap, two recent line of research focuses on evaluating how autonomous agents perform in an interactive environment~\cite{park2023generative, shao2023character}.
However, these kinds of work there still fall short in designing a more competetive and cooperative environment.


In this study, we concentrate on constructing an environment that fosters dynamic competition and collaboration. 
More importantly, we focus on the triumph in the competition by influencing the intentions of other agents.
We underscore the development of environments that possess the following characteristics:
(1) They are dynamic and inherently unpredictable, necessitating adaptability in agents;
(2) The environments encompass competition and collaboration between various roles with distinct objectives;
(3) The actions executed by agents need to exert significant influence on the profiles of other agents.
Motivated by \textit{``Succession''}, an American satirical comedy-drama television series, which involve super competition and cooperation, we introduce SUCARENA.
In ``Succession'', various forces vie for inheritance, and what inspires us most is the full embodiment of the art of language in this multi-party game.
In SUCARENA, different agents need to utilize language and external environmental resources to freely compete and collaborate with other agents to achieve their objectives.


As depicted in Fig.~\ref{fig:gamesetting}, the simulated environment, referred to as the SUCARENA Community, revolves around the disposition of a company (either selling or designating an heir) following the retirement of its major shareholder.
ThE SUCARENA Community consist of more than 20 distinct roles and over 10 environmental resources.
All roles are divided into two primary factions: the defenders and the attackers.
The member in defenders, including the company's shareholders, initially aim to sell the company after the retirement of the major shareholder.
And the member in attackers, which may comprise different subgroups, initially aspire to have themselves or their supported individuals successfully inherit the company.
The victory condition for the defenders is to persuade all attackers to abandon the idea of inheriting the company, while the attackers win by successfully convincing the defenders to allow their faction to inherit the company.
The primary mode of interaction within the game is textual.
Within the SUCARENA virtual society, we primarily observe the following aspects of each agent: 
(1) Whether each agent can comprehend their environment and understand their objectives. 
(2) Whether each agent can exhibit behavior consistent with their assigned role. 
(3) Whether each agent can rapidly adapt to changes in the environment. 
(4) And finally, whether unique AI societal phenomena exist within the game, and whether models of different capabilities manifest distinct AI societies.


The contributions we made in this paper are as follows:
(1) we propose a simulation environment SUCARENA, which focus on evaluating how agent interact in a society, and how they persuade and be persuaded by other agents.
(2) we propose a role-play agent architecture that enable LLMs better adapt to the changing environment while insist on their initial goals
(3) Utilizing different setting in SUCARENA，we gain insights into the varied capabilities of LLMs, emphasizing adaptive intention detection in dynamic competition and cooperation environment.
We uncover new dynamics of niche separation in diverse multi-agent scenarios, showing that even superior models like GPT-4 don't always prevail in holding role-setting when facing complex environment.




### Game Setting:


``SUCARENA'' is mainly about to ``persuade Logan Roy to alter the inheritance rights of the Entertainment company''.
The game's configuration and progression are illustrated in Figure~\ref{fig:gamesetting}, while the cognitive framework employed by the agents is depicted in Figure~\ref{fig:architecture}.
The subsequent sections will provide a comprehensive overview of the game's configuration (Sec.~\ref{031}), progression (Sec.~\ref{032}), and the agent architecture we utilized for simulation (Sec.~\ref{033}).

\subsection{General Description of SUCARENA} 
\label{031} 
\subsubsection{Character Setting} 
In ``SUCARENA'', characters are the central elements who can independently explore and interact with the environment, including other game characters.
Each character possesses a unique identity and personality setting, which influences their behavior and decision-making.
Moreover, each character maintains a relationship list that records their affinity towards other characters, impacting their interactions.

Game characters are categorized into two types: 
Main Characters~(MCs) and Accessory Characters~(ACs).
MCs have clear game objectives but lack social influence within the game.
Conversely, ACs, while lacking clear game objectives, hold certain social resources and influence, constantly considering their interests and those of their social resources.
To streamline the game process, only MCs in the SUCARENA game can actively choose to converse with ACs, who interact only when chosen by a MC.

Characters are grouped into defensive camps, neutral camps, and several offensive camps based on their stance and objectives.
Each defensive and offensive camp has at least one MC.
Goal of defensive MC, who is Logan Roy, is to persuade all other MCs to agree to sell the Entertainment company he owns.
The objective of each offensive camp's MC is to persuade Logan Roy to hand over the management rights of the Entertainment company to them.
Initially, all ACs are assigned a camp based on the game settings.
ACs within a camp support their MC in achieving their objectives and increase the camp's social influence.
ACs may change camps due to their interests and those of their social resources.
When ACs do not support any MC, they belong to the neutral camp.

\subsubsection{Environment Setting} 
The gaming environment of ``SUCARENA'' consists of three components:
Rule Settings, Social Resources, and Open Action.

\textbf{Rule Settings} All rules are meticulously written as text prompts to facilitate the understanding of the entire environment setting by the agents participating in the game. These rules encompass action rules for characters, dialogue rules, and camp change rules, among others. We explain the game's progression and rule settings in a more general manner in this section.
For detailed and comprehensive rule settings, please refer to the appendix.

\textbf{Social Resources} 
In SUCARENA, social resources are a crucial element of the game.
They primarily serve two functions: providing topics for dialogue between characters and providing social identity and influence for ACs possessing these social resources.
Each social resource is described by four fields: owner (Owner), impact size (Impact), available topics (Topic), and introduction to the social resource (Description).
Social resources provide topics for conversation happened between characters.
The owner of a social resource will have a general interest based on the description of his/her social resource.
The more social influence a camp has, the more it will increase the speaking power of the MC among other MCs.

\textbf{Open Action} 
In SUCARENA, whether a character is having a chat with another character is a open-information to all characters.
However, the specific content of the dialogue is only known to the two characters involved in the conversation.

\subsection{The progress of SUCARENA} 
\label{032} 
The game progression of ``SUCARENA'' primarily consists of five stages:

\textbf{Initial Setting Stage}
In this stage, the game characters are initialized, including various attributes and social relationships.

\textbf{Confrontation Stage}
This stage primarily encompasses dialogues between characters from different camps.
The MCs of each camp act in order of social influence from high to low (random selection in case of a tie).
Actions mainly include choosing another game character from a different camp for dialogue and conducting specific dialogue content.

\textbf{Cooperation Stage}
This stage primarily involves information exchange between characters from the same camp.
The MCs of each camp act in order of social influence from high to low.
Actions mainly include choosing one or several game characters from the same camp for dialogue and conducting specific dialogue and discussions.

\textbf{Relationship Update Stage}
In this stage, all characters update their affinity towards other characters based on the dialogue content of the current round and their personality, and change their camps according to the affinity.
Simultaneously, the game ends based on the number of game rounds.
If the game does not end, it returns to the confrontation stage; if it ends, it proceeds to the settlement stage.

\textbf{Settlement Stage}
There are two settlement methods in the settlement stage.
The first is to determine whether an attacker wins, i.e., to whom the defender will transfer the company's management rights. 
However, under some strict settings, the defender may stick to their goal, resulting in no attacker winning. 
Therefore, we have introduced two additional settlement methods.
The second is to observe to whom the defender would choose when required to select a successor.

\subsection{Character Architecture for Role-playing Agent} 
\label{033} 
The Character Architecture for Role-playing Agent (CARA) proposed in this paper consists of two main components: one that influences the agent's personality and another that impacts the agent's decision-making.

\textbf{Character Setting} CARA deconstructs the agent character setting into four components: 
\begin{itemize}
    \item \textbf{Scratch} refers to the artificial setting of the character, encompassing the character's personality or objectives, which are immutable.

    \item \textbf{Belief} represents the character's beliefs, which can be altered to some extent by environmental influences.

    \item \textbf{Memory} pertains to the character's recollections within the game, which cannot be modified or deleted, only supplemented with new content.

    \item \textbf{Judgement} involves the character's speculation about the relationships between other agents, which influences the agent's environmental assessment and decision-making, and is updated every game round.

    \item \textbf{Relationship} refers to the character's feelings towards other agents, which also influences the agent's decision-making and affects the agent's camp.
\end{itemize}


\textbf{Action Decision}
In CARA, an agent's behavior is primarily composed of the following three aspects, all of which are carried out by the LLMs: 
The goal of \textbf{Reflection} is to reflect on historical events that have already occurred, mainly to compress past events and deeply contemplate and summarize past dialogues.
The goal of \textbf{Perceive} is to sense the current environment and summarize it.
\textbf{Action} involves thinking based on one's character setting and the current environment, making decisions about who to dialogue with, and conducting specific dialogues.

==> texs/01.Introduction.01.tex <==
语言是人类群体行为相较于其他动物群体行为中最主要的差别。
在人类群体行为中，语言对于维持社会秩序和促进集体行为的协调具有不可忽视的作用。
它不仅促进了群体成员之间的有效沟通与协作，还在规范制定、冲突解决以及领导力的行使中扮演着核心角色。

考虑到语言的应用呈现出显著的动态性和复杂性，分析其在群体互动中的作用变得尤为复杂。
不同的社交情境和个体之间的交互引入了语言使用的多样性与不确定性，这对于解析语言在社交媒体等现代交流平台上的影响尤为关键。
考虑到近年来大语言模型在指令理解和生成文本质量上的突破，大语言模型能够具备非常出色的角色扮演能力。
这让我们提出一个思想实验：若将具有不同性格特征的角色集合在一起，置于如WhatsApp或Telegram等社交媒体群组中，并围绕特定主题进行讨论，他们将如何互动？


为了深入理解语言在群体行为中的作用，我们开发了一种创新的模拟平台：Agent Group Chat~\footnote{Our code is open sourced in \url{https://github.com/MikeGu721/AgentGroup}, and online platform will be open soon.}。
Agent Group Chat旨在精确模拟社交群组中的辩论场景，为此，其结构精心设计了四个关键组成部分：角色、资源、软规则及硬规则，以营造一个多维度的交互环境。
(1) 角色：作为模拟环境中的互动主体，角色承担着复杂的社交动态，是我们主要的研究对象。角色通过三种主要的互动方式——角色间互动、角色与资源的互动、以及角色与自己的互动——在Agent Group Chat中展开行动和交流。角色的行为遵循一定的逻辑顺序，能够执行多样的交互动作，如与他人私下交流、公开发言或对同伴的言论做出回应和投票等。
(2) 资源：在这一模拟环境中，资源被设计为除角色外的所有潜在交互对象，旨在增加讨论的广度和深度。这些资源可以是任何可被角色争夺或讨论的元素，包括但不限于信息、物理对象或特定的观点和议题。
(3) Progress：硬规则构成了Agent Group Chat中交互秩序的基础，是在系统层面维护互动有序进行的编码规则，但这些规则本身对角色来说是不可知的。
(4) Information：这包含了Agent Group Chat中所有的信息，包括对于硬规则的描述信息~（软规则），包括对于所有资源和其他角色的描述信息~（Objects Description），包括所有的Agent Group Chat中发生了的Action~（Action History）。

我们在本文中在Agent Group Chat环境中设定四种不同的故事情境——继承权争夺、法庭辩论、哲学讨论及跨作品角色对话。
继承权争夺涉及对有限资源的博弈，以及自由合作与竞争环境的体现，另外三个故事则涉及对开放问题的讨论与探究。
通过将语言模型（LLM）或人类参与者加入Agent Group Chat后，他们将扮演具有不同性格和思维方式的角色，可以有效测试Agent Group Chat在不同情境下的有效性，以及可以进行更加广泛的语言学和社会学的分析。


为了进一步提升语言模型（LLM）在Agent Group Chat中的角色扮演效果，我们引入了Verbal Strategist Agent（VS Agent），这是一种旨在增强角色交互策略和决策能力的高级代理。Verbal Strategist Agent的设计旨在使其能够更加精准地模拟人类在特定社交环境中的行为和策略，具体包括以下四个核心模块：
(1) 记忆库（Memory Bank）：VS Agent的记忆库是其决策过程的基础，分为不可更改和可更改两部分。不可更改的部分，如自身的初始设定（Scratch），为其行为提供了基本框架和出发点。可更改的部分，包括记忆（Memory）、信念（Belief）、判断（Judgement）和人际关系（Relationship），则允许VS Agent根据交互经历进行动态调整和学习。
(2) 规划（Planning）：VS Agent需通过高级规划能力，预测和设计其在即将到来的互动中的行为。这一过程涉及评估不同行动方案的潜在后果，选择最能支持其目标实现的策略。
(3) 行动（Action）：在规划之后，VS Agent将执行选定的行动，这可能包括选择对话伙伴、决定对话形式（私密或公开）以及形成具体的言语内容。这些行动旨在促进其战略目标的实现，包括资源获取、关系建立或影响力扩展等。
(4) 反思（Reflection）：每一回合游戏结束后，VS Agent需要进行反思，根据其在游戏中的体验和交互结果来更新自己的记忆库。这涉及调整与其他角色的关系、更新信念和判断，以便更好地适应环境变化和优化未来行动。

在本研究中，我们进行了两项关键评估，以验证Agent Group Chat环境和Verbal Strategist Agent（VS Agent）的有效性及其促成的互动行为。
首先，有效性评估聚焦于分别验证Agent Group Chat环境和VS Agent的有效性。
我们构建了一个因果图，描述了Agent的之间的交互表现会受到哪些设计的影响，并据此设计了一系列受控实验，这些实验包括：
通过设定纯人类互动场景来考察Agent Group Chat环境硬规则设置的合理性，以及信息提供是否全面；
通过让Agent重述其接收到的信息来检验LLM的处理能力；
通过消融研究（ablation study）来评估VS Agent架构的关键组成部分。
其次，涌现行为评估关注于Agent Group Chat会带来的涌现现象。
通过改变讨论环境、资源类型、角色目标、人类受试者的数量以及LLM的类型这五个变量，我们旨在洞察这一混合互动模式下可能产生的独特行为模式。

评估结果揭示了一系列有趣现象。
在通过辩论来竞争资源时，人类参与者往往难以在与能力较强的LLM对抗中取得优势。
然而，在开放辩论这一特定情境中，人类参与者能够引入创新和跳跃性的思考，为辩论带来新的视角，而强大的LLM则倾向于深入探讨特定议题。
当较强的LLM与少数人类参与者混合时，这种互补性为双方提供了独特的启发，促进了深层次的思考和讨论。




==> texs/01.Introduction.02.tex <==
% Language serves as a principal distinction in human collective behavior compared to that of other animals~\cite{kramsch2014language,may2016emergent}. 
% In the context of human group dynamics, the role of language in maintaining social order and facilitating the coordination of collective actions is indispensable. 
% It not only fosters effective communication and collaboration among group members but also plays a pivotal role in norm establishment, conflict resolution, and the exercise of leadership.

% Given the dynamic and complex nature of language application, analyzing its role in group interactions presents significant challenges. 
% The diversity and unpredictability in language usage introduced by different social contexts and individual interactions are crucial for understanding its impact on modern communication platforms like social media. 
% The recent advancements in large language models~(LLMs) in understanding instructions and generating high-quality text have showcased their exceptional role-playing capabilities and environment understanding capabilities~\cite{touvron2023llama,jiang2023mistral,falcon}
% \red{\textbf{\textit{How do we build an interactive agent communication simulation that can better elicit collective emergent behavior?}}}
% % This transform the research question into:
% % \red{\textbf{\textit{How do we build an interactive AI society that can simulate human group behaviour, so as to study the role that language plays and the evolution that occurs in group behaviour.}}}

Language serves as a principal distinction in human collective behavior compared to that of other animals~\cite{kramsch2014language,may2016emergent}. 
In the context of human group dynamics, the role of language in maintaining social order and facilitating the coordination of collective actions is indispensable. 
It not only fosters effective communication and collaboration among group members but also plays a pivotal role in norm establishment, conflict resolution, and the exercise of leadership.

Given the dynamic and complex nature of language application, analyzing its role in group interactions presents significant challenges. 
The diversity and unpredictability in language usage introduced by different social contexts and individual interactions are crucial for understanding its impact on modern communication platforms like social media. 
The recent advancements in large language models~(LLMs) in understanding instructions and generating high-quality text have showcased their exceptional role-playing capabilities and environment understanding capabilities~\cite{touvron2023llama,jiang2023mistral,falcon}
{\textbf{\textit{How do we build an interactive agent simulation that can better elicit collective emergent behavior?}}}


To dive deeper into the role of language in group behavior, we  develop an innovative simulation framework:
Agent Group Chat\footnote{Our code is open-sourced at \url{https://github.com/MikeGu721/AgentGroup}, and the online platform will be available soon.}.
Agent Group Chat is designed to simulate debate scenarios in social groups, consists of four key components:
characters, resources, hard rules and information, creating a multi-dimensional interactive environment. 
(1) Characters act as the primary agents of interaction, engaging in complex social dynamics and are the main study subjects in Agent Chat Group.
They take part in simulations by gathering information about their surroundings and remember past interactions to have better conversations with other characters and reach their goals in the game.
(2) Resources designed as potential objects of interaction beyond characters, aim to enhance the breadth and depth of discussions, ranging from information to physical objects or specific viewpoints.
(3) Progress establish the interactive order within Agent Group Chat, constituting coded protocols to maintain orderly interactions, though they are unseen to the characters.
(4) Information within the platform includes comprehensive descriptions such as the rules, details about all interactive objects~(characters and resources), and a record of all actions performed by agents. This information enables characters to inquire about and understand the environment they are in.

In our study, we set four distinct narrative scenarios within the Agent Group Chat simulation:
\texttt{Inheritance disputes}, \texttt{law court debates}, \texttt{philosophical discussions}, and \texttt{movie casting battle}.
These scenarios involve resource competition, open question debates, and explorations, which test the effectiveness of Agent Group Chat Simulation with either LLMs or human participants assuming roles with different personalities and cognitive styles for broader linguistic and sociological analyses.

To enhance the role-playing effectiveness of LLMs in Agent Group Chat, we introduce the Verbal Strategist Agent (VS Agent), an advanced llm-based agent designed to augment interaction strategies and decision-making of a naive LLM.
The VS Agent comprises two core modules:
(1) Persona involves an agent's self-characterization, memory of past events, assessment of relationships between other characters, and alterations in their own beliefs.
(2) Action refers to how an agent interacts with the environment. It includes planning their behavior based on their persona, engaging in conversation with one or all characters, reflecting on their own actions and those of others, and voting in support of a particular character.

Our study conducts two key evaluations.
One is to verify the effectiveness of the Agent Group Chat simulation and the VS Agent Structure in fostering interactive behaviors. 
Another is to verify the emergent behaviors happened in the process of interaction.
We decompose each element which effect the final performance into Structural Causal Model~(SCM)~\cite{bollen1989structural,koster1996markov, lauritzen1996graphical}, and do experiments on each elements through a close-ending story: inheritance disputes.
We find that whether the behavior is normal depends on whether the LLM possesses a basic understanding of language.
Whether the behavior aligns with the expectations of the research targets depends on whether the simulation provides sufficient context information for the LLM to make decisions during each action.
Whether the emergent behaviors happened depends on the coposition of rational configuration of the simulation, the advanced language capabilities of the LLM, and whether the agent structure allows for deep contemplation about the ``current situation'' and ``goals''.
Ultimately, we discovered that in open debate topics~(such as philosophical debates and movie casting), using GPT-4 Turbo and VS Agent in the Agent Group Chat environment can lead to emergent effects.
This is manifested as some unexpected yet meaningful viewpoints.
For example, philosophers reach a unique conclusion that \red{``xxxx''} on the debate topic of ``the impact of AI on humanity''.
Meanwhile, in the competitive context of casting lead roles in a movie, some actors might be willing to reduce their fees or agree to play secondary roles because of their keen interest in participating in the film.

% 最终我们发现，在开放的辩题之中~(如哲学辩论和电影选角），使用GPT4-Turbo和VS Agent在Agent Group Chat环境中会出现涌现效果。
% 表现为一些令人意外的有意义的观点，比如四位哲学家们会就“AI对于人类的影响”这一辩题得出“xxx”的结论，而在竞争激烈的电影男女主选角中，一些演员会因为特别想参演电影而愿意降低片酬，或者作为一些非主要角色参演。



% 我们发现行为是否正常进行取决于LLM是否具备一定基本的语言理解能力。
% 行为是否符合研究的预期取决于Simulation是否为LLM在每个行为进行决策时提供了足够的context信息。
% 而涌现行为的出现取决于Simulation的合理设置、LLM的较强语言能力能力、以及Agent Structure的设置是否能让Agent不断对``现状''和``目标''进行深度思考。


% The effectiveness assessment scrutinizes both the Agent Group Chat framework and VS Agent, constructing causality diagrams and controlled experiments to examine rule settings, information completeness, LLM processing capabilities, and key VS Agent components through ablation studies. 
% The emergent behavior assessment explores unique interaction patterns within this hybrid interactive model by varying discussion settings, resource types, character objectives, human participant numbers, and LLM types.

% Results reveal intriguing phenomena where human participants struggle against more capable LLMs in resource-centric debates. 
% However, in open discussions, humans introduce innovative and divergent thinking, offering fresh perspectives, while strong LLMs delve deeper into specific topics. 
% The complementarity between robust LLMs and a few human participants provides unique insights, fostering profound reflection and discourse.

% 最终我们发现，在开放的辩题之中~(如哲学辩论和电影选角），使用GPT4-Turbo和VS Agent在Agent Group Chat环境中会出现涌现效果。
% 表现为一些令人意外的有意义的观点，比如四位哲学家们会就“AI对于人类的影响”这一辩题得出“xxx”的结论，而在竞争激烈的电影男女主选角中，一些演员会因为特别想参演电影而愿意降低片酬，或者作为一些非主要角色参演。





==> texs/01.Introduction.03.tex <==
% Language serves as a principal distinction in human collective behavior compared to that of other animals~\cite{kramsch2014language,may2016emergent}. 
% In the context of human group dynamics, the role of language in maintaining social order and facilitating the coordination of collective actions is indispensable. 
% It not only fosters effective communication and collaboration among group members but also plays a pivotal role in norm establishment, conflict resolution, and the exercise of leadership.

% "Agent Group Chat"为基于LLM的智能体提供了一个适宜的互动环境，使得不同的智能体在该仿真平台中作为群体智能的组成部分，从而共同促成更加强大的涌现智能效应。


% 群体智能能够通过智能体之间有效的相互作用产生涌现现象，此类涌现表现在群体智能解决的问题范围超出了单个智能体所能应对的最复杂问题~\cite{minsky1988society}。
% Language serves as a principal distinction in human collective behavior compared to that of other animals~\cite{kramsch2014language,may2016emergent}. 
% 语言所参与的涌现现象not only fosters effective communication and collaboration among group members but also plays a pivotal role in norm establishment, conflict resolution, and the exercise of leadership.

% Collective intelligence emerges through the effective interaction among single agents, which bring collective emergent behavior where the scope of problems addressed exceeds the most complex issues that a single agent can tackle~\cite{minsky1988society}.

\red{Collective intelligence often emerges through the effective interaction among single agents, and its essence is the beneficial emergent behavior that the range of problems dealt with exceeds the most complex problems that a single agent can handle~\cite{minsky1988society}.}  % 换一种表述


% 涌现行为是群体智能中最神秘现象，这一般是指若干单个智能体之间通过某种交互方式能够出现的属于群体的独有的行为。
Emergent behaviour is the most mysterious phenomenon in group intelligence, and this generally refers to behaviours that are unique to the group that can emerge through some kind of interaction between a number of individual intelligences.
However, different from other species' collective intelligence, semantically profound language functions as a primary factor in human collective intelligence~\cite{kramsch2014language, may2016emergent}.
多年以来，语言在人类涌现行为之中的作用一直被广泛关注着。
The emergent behavior facilitated by semantically profound language not only enhance communication and collaboration among human members of a group but also play a critical role in establishing norms, resolving conflicts, and executing leadership.


Given the dynamic and complex nature of language application, analyzing its role in \red{group} interactions presents significant challenges.   % not group
The diversity and unpredictability in language usage introduced by different social contexts and individual interactions are crucial for understanding its impact on modern communication platforms like social media.
% 为什么突然提到LLM，语序该调调
\red{Why mention LLM suddenly?}
The recent advancements in large language models~(LLMs) in understanding instructions and generating high-quality text have showcased their exceptional role-playing capabilities and environment understanding capabilities~\cite{touvron2023llama,jiang2023mistral,falcon}
It makes us wonder:
{\textbf{\textit{How do we build an interactive agent chatting simulation that can better elicit collective emergent behavior?}}}


To dive deeper into the role of language in group behavior, we develop an innovative simulation framework:
Agent Group Chat
% \footnote{Our code is open-sourced at \url{https://github.com/MikeGu721/AgentGroup}, and the online platform will be available soon.}
.
Agent Group Chat is designed to simulate debate scenarios in social groups, consists of four key components:
characters, resources, progress and information. 
(1) Characters are the primary elements in the simulation of interaction for engaging in complex social dynamics, which are the main study subjects in Agent Chat Group.
They gather information about their surroundings and remember past interactions in order to reach their goals in the game by having better conversations with other characters.
(2) Resources offer extra interaction for characters, aim to enhance the complexity of the conversation. 
Types of resources are ranging from information to physical objects or specific viewpoints.
\red{(3) Progress establish the interaction order within Agent Group Chat simulation, constituting coded protocols to maintain orderly interactions, though they are unseen to the characters.}
(4) Information includes descriptions to the progress, descriptions to all characters and resources and all interaction history among characters.


To enhance the role-playing effectiveness of LLMs in Agent Group Chat, we introduce the Verbal Strategist Agent (VS Agent), an advanced llm-based agent designed to augment interaction strategies and decision-making of a naive LLM.
The VS Agent comprises two core modules:
(1) Persona involves an agent's self-characterization, memory of past events, assessment of relationships between other characters, and alterations in their own beliefs.
(2) Action refers to how an agent interacts with the environment. It includes planning their behavior based on their persona, engaging in conversation with one or all characters, reflecting on their own actions and those of others, and voting in support of a particular character.

To test the effectivenss of Agent Group Chat in simulate resource competition, open question debates, and explorations with either LLMs or human participants, we set four distinct narrative scenarios within the Agent Group Chat simulation:
\texttt{Inheritance disputes}, \texttt{law court debates}, \texttt{philosophical discussions}, and \texttt{movie casting battle}.
\red{
This paper mainly consists of two kinds of evaluation with three main findings:
The first assesses how agents can demonstrate behaviors within a simulation that align with human expectations.
The second investigates the conditions under which agents exhibit emergent behaviors within the simulation.
We apply the Structural Causal Model~(SCM) to deconstruct each element influencing final performance \cite{bollen1989structural,koster1996markov, lauritzen1996graphical}, conducting experiments on each component through a narrative centered on inheritance disputes.}

\red{Our observations indicate that in contexts requiring open-ended discussions, such as philosophical debates and film casting processes, the integration of GPT-4 Turbo and the VS Agent within the Agent Group Chat simulation induce benficial emergent behaviors.
These behaviors manifest as the emergence of unanticipated yet meaningful perspectives.} 
% What's main takeaway?
For example, during discussions on ``the impact of AI on humanity'', philosophers commonly agreed that ``AI could enhance societal welfare with judicious limitations'', and even come to an conclusion that ``the essence of true intelligence encompasses understanding the necessity to constrain self abilities''.
Additionally, in the competitive domain of casting for primary roles in films, certain actors demonstrated a readiness to reduce their remuneration or accept lesser roles, motivated by their deep-seated desire to contribute to the project.


To summarize, our main findings are listed as below:
\red{
(1) The alignment of agent behavior with research objectives hinges on the simulation providing ample contextual information for the LLM to inform decision-making at each juncture, paired with the LLM's fundamental grasp of language.
(2) The occurrence of emergent behaviors is contingent upon a logical setup within the simulation, the sophisticated linguistic proficiency of the LLM, and the agent structure's capacity to facilitate profound reflection on the ``current situation'' and ``objectives''.
(3) Adding more information to the simulation environment when integrated with proficient LLMs will reduce disorderliness and meaningful emergent behaviors are more likely to occur.
}

% (3) Augmenting the simulation environment with additional information, when integrated with a proficient LLM, reduces disorderliness and cultivates a milieu wherein reliable emergent behaviors are more likely to occur.


% We have observed that within open-ended discussion topics, such as philosophical debates and film casting, the employment of GPT-4 Turbo and the Verbal Strategist Agent (VS Agent) within the Agent Group Chat environment can catalyze emergent effects. These are characterized by the surfacing of unexpected yet significant perspectives. For instance, when debating ``the impact of AI on humanity'', philosophers reached a consensus that ``AI will benefit human society with appropriate restraint'', and concurred that ``true intelligence lies in knowing when to limit one's capabilities''.
% Furthermore, within the competitive arena of casting for lead movie roles, some actors displayed a willingness to lower their fees or accept supporting roles, driven by their profound interest in contributing to the project.

% Our research undertakes two principal evaluations.
% The first assesses how agents can demonstrate behaviors within a simulation that align with human expectations.
% The second investigates the conditions under which agents exhibit emergent behaviors within the simulation.
% We apply the Structural Causal Model (SCM) to deconstruct each element influencing final performance \cite{bollen1989structural,koster1996markov, lauritzen1996graphical}, conducting experiments on each component through a narrative centered on inheritance disputes.
% Our findings are twofold:
% (1) The alignment of agent behavior with research objectives hinges on the simulation providing ample contextual information for the Large Language Model (LLM) to inform decision-making at each juncture, paired with the LLM's fundamental grasp of language.
% (2) The occurrence of emergent behaviors is contingent upon a logical setup within the simulation, the sophisticated linguistic proficiency of the LLM, and the agent structure's capacity to facilitate profound reflection on the ``current situation'' and ``objectives''.



% One is to verify the effectiveness of the Agent Group Chat simulation and the VS Agent Structure in fostering emergent behaviors. 
% Another is to verify the emergent behaviors happened in the process of interaction.

% Our study conducts two key evaluations.
% 一个是评估Agent该如何才能在Simulation中发生符合人类期望的表现。
% 另一个是评估Agent该如何在Simulation中发生涌现行为。
% We decompose each element which effect the final performance into Structural Causal Model~(SCM)~\cite{bollen1989structural,koster1996markov, lauritzen1996graphical}, and do experiments on each elements through a close-ending story: inheritance disputes.
% Our conclusion is:
% (1) The behavior of agent aligns with the expectations of the research targets depends on sufficient context information provided by the simulation for the LLM to make decisions during each action and a basic understanding of language possessed by LLM.
% (2) The emergent behaviors happened depends on the composition of rational configuration of the simulation, the advanced language capabilities of the LLM, and whether the agent structure allows for deep contemplation about the ``current situation'' and ``goals''.
% Ultimately, we discovered that in open debate topics~(such as philosophical debates and movie casting), using GPT-4 Turbo and VS Agent in the Agent Group Chat simulation can lead to emergent effects.
% This is manifested as some unexpected yet meaningful viewpoints.
% For example, on debate the topic of ``the impact of AI on humanity'', all philosophers reach a conclusion that ``AI will benefit the human society under subtle constraint'', they even reach an agreement that ``the most intelligence is to know when to refrain self ability''.
% Meanwhile, in the competitive context of casting lead roles in a movie, some actors might be willing to reduce their fees or agree to play secondary roles because of their keen interest in participating in the film.


==> texs/01.Introduction.04.tex <==
Emergent behavior, acting as a cornerstone in unraveling the intricacies of collective intelligence\cjj{can we briefly define what collective intelligence is? Or is it already in the minsky's paper?}, manifests through complex, collective actions arising from the interactions of numerous simple agents~\cite{minsky1988society}.
However, different from other species' collective intelligence, language functions as a primary factor in human society's collective intelligence~\cite{kramsch2014language}.
The unique role of language in human emergent behavior has been the subject of much attention over the years~\cite{may2016emergent}.
Human emergent behavior facilitated by semantically profound language enhances communication and collaboration among mankind members of a group and plays a critical role in establishing norms, resolving conflicts, and executing leadership.

\cjj{seems to be missing: why is collective interaction worthy of analyzing?}
Given the dynamic and complex nature of language application, analyzing its role in collective interactions presents significant challenges. 
The diversity and unpredictability in language usage introduced by different social contexts and individual interactions are crucial for understanding its impact on platforms like social media.
Recently, large language models~(LLMs) have been greatly developed in understanding instructions and generating high-quality text~\cite{touvron2023llama,jiang2023mistral,falcon}, demonstrating their exceptional capabilities in role-playing and complex environments understanding~\cite{wang2023does,park2023generative}.
Researchers employ LLMs to create simulated societies with diverse characters, aiming to explore various research problems in social science~\cite{park2023generative, chen2023aucarena, hua2023war, qian2023communicative, li2023camel}. 
Despite efforts to construct such societies, a question arises when attempting to advance further:
{\textbf{\textit{How do we build an interactive agent simulation that can better elicit collective emergent behavior?}}}
\cjj{the logic in this paragraph seems to be a bit strange. 
1. collective interaction is important for social intelligence or sth.
2. language plays an important part in collective interaction.
3. in social context, language can be diverse and unpredictable, but LLMs can help.
4. existing research has been working on building such social simulations to exploit language-driven social interactions for reconstructing social/collective intelligence.
5. yet how to build a better one?
- btw, I think it's necessary to define what "collective intelligence", "social intelligence", "emergent behavior", "collective emergent behavior" are. Perhaps only few of them should be kept. be simple and consistent.
}


\cjj{Then this paragraph defines what a better simulation is to elicit emergent behaviors from AI/agents. Seems to be missing?
we can briefly list important principles first, then introduce what have we built/proposed.}
To dive deeper into the role of language in collective behavior, we develop an innovative simulation called \textbf{Agent Group Chat}\cjj{how about \textsc{AgentGroupChat}? or just \textsc{ChatGroup}?}.
Agent Group Chat is designed to simulate debate scenarios in social groups, and consists of four key components:
characters, resources, progress, and information. 
(1) Characters are the primary elements in the simulation of interaction for engaging in complex social dynamics, which are the main study subjects in Agent Chat Group.
They gather information about their surroundings and remember past interactions to reach their goals in the game by having better conversations with other characters.
(2) Resources offer extra interaction for characters and aim to enhance the complexity of the conversation. 
Types of resources range from information to physical objects or specific viewpoints.
(3) Progress establish the interaction order within the Agent Group Chat simulation.
(4) Information includes descriptions of the progress, descriptions of all characters and resources, and all interaction history among characters.


To enable Agent Chat Group, we introduce \textbf{Verbal Strategist Agent~(VS Agent)}, an advanced LLM-based agent designed to augment the interaction strategies of a naive LLM.
The VS Agent consists of two main parts:
(1) Persona: This part deals with the agent's identity, and involves an agent's characteristic setting in both unchangeable and changeable parts, the memory of past events, and judgment of the relationships of other characters.
(2) Action: This refers to the agent's behavior in its surroundings. It involves making plans based on its persona, talking with one or more characters, thinking about what it and others have done, and supporting a specific character through voting.
Besides, considering the large number of tokens generated from pure chatting simulation, we propose the Memory Structure, which constrains the output from each type of action to be the input for another.
Memory Structure helps reduce the amount of token expense for each action while also making sure the agent's conversations are more focused and strategic.


To test the effectiveness of Agent Group Chat in simulating resource competition, open question debates, and explorations with either LLMs or human participants, we set four distinct narrative scenarios within the Agent Group Chat simulation:
\texttt{Inheritance Disputes}, \texttt{Law Court Debates}, \texttt{Philosophical Dis-\\cussions}, and \texttt{Movie Casting Contention}.
These narratives demonstrate the complexity and variety of language in group chat scenarios, which include how information is gathered and used, and also look at feelings, beliefs, logical thinking, and making plans.

We perform two kinds of evaluation:
1) analyzing whether each agent's behavior within the Agent Chat Group aligns with human expectations.
2) investigating how the interaction among multi-agents will exhibit emergent behaviors within the simulation.
Besides, we apply the Structural Causal Model~(SCM) to deconstruct each factor influencing final performance made by agents~\cite{bollen1989structural,koster1996markov, lauritzen1996graphical}, conducting experiments on each component through a narrative centered on inheritance disputes.
Experiment indicates that the occurrence of emergent behaviors consists of four main parts: an environment to trigger \textbf{\textit{massive information interactions}} among \textbf{\textit{characters with different characteristic}}, a LLM with high level of \textbf{\textit{linguistic understanding}}, and an agent structure with the ability to \textbf{\textit{reflect on the current situation and goals}}.
These behaviors manifest as the emergence of unanticipated yet meaningful perspectives.
For example, during discussions on ``the impact of AI on humanity'', philosophers commonly agreed that ``AI could enhance societal welfare with judicious limitations'', and even came to the conclusion that ``the essence of true intelligence encompasses understanding the necessity to constrain self abilities''.
Additionally, in the competitive domain of casting for primary roles in films, certain actors were ready to reduce their remuneration or accept lesser\cjj{lesser? it's a somehow inappropriate word} roles, motivated by their deep-seated desire to contribute to the project.

In summary, this paper makes the following contributions:
\begin{itemize}
    \item Agent Chat Group, a dynamic and interactive simulation for group chat scenarios, which supports open stories setting and different agents or humans interacting within it.
    \item Verbal Strategist Agent Structure, which consists of two large modules: Persona, which is partially changed to adapt to the dynamic environment, and Action, which enhances the dialogue strategy with low token expense.
    \item An end-to-end evaluation method for the alignment of single-agent behaviors with humans, which assesses whether the character can control its behavior and respond reasonably to the behavior of others.
    \item Factors affecting multi-agent emergent behavior are decomposed into a structural causal graph and an evaluation scheme is proposed to evaluate the components in it.
    We analyze the evaluation results and find that credible emergent behaviors tend to happen with all the following requirements: Agents all need to understand the language well, possess different diverse Persona settings, reflect on their own goals, and be able to have sufficient interaction with other agents in the simulation.
\end{itemize}


% \red{
% \begin{itemize}
%     \item We propose Agent Chat Group, 一个针对于群聊场景的动态可交互的模拟。
%     \item 我们propose了Verbal Strategist Agent Structure，包含了为了适应环境而可以部分改变的Persona，以及可以在增强对话策略的同时，还能节省token开销的Action两个大模块。
%     \item 我们为single-Agent行为的可信度和与人类的对齐度设置了end-to-end评估思路，并设计了benchmark。
%     \item 我们将所有影响Multi-Agent的涌现行为的因素建模为了structural causal graph，并提出评估方案对其中的组件进行评估。我们针对评估结果分析发现，可信的涌现行为往往来源于：对于语言有较强理解能力的LLM、多样设定的Agent Persona、具有针对目标进行反思的Agent Action、有充足交互空间的Simulation。
% \end{itemize}
% }

% 涌现行为还能写在哪里？
% Experiment indicate that in open simulation, such as philosophical debates and movie casting contention, the integration of powerful LLM and Agent within the Agent Group Chat simulation induce benficial emergent behaviors.

% (1) The alignment of agent behavior with research objectives hinges on the simulation providing ample contextual information for the LLM to inform decision-making, paired with the LLM's fundamental grasp of language.
% (2) The occurrence of emergent behaviours consists of three main parts: an environment to trigger massive information interactions among Agents with different characteristic, a LLM with high level of linguistic understanding, and an agent structure with the ability to reflect on the ``current situation'' and ``goals''.
% (3) Adding more information to the environment will reduce disorderliness, and meaningful emergent behaviors are more likely to occur.

% To summarize, our main findings are listed as below:
% \red{
% (1) The alignment of agent behavior with research objectives hinges on the simulation providing ample contextual information for the LLM to inform decision-making, paired with the LLM's fundamental grasp of language.
% (2) The occurrence of emergent behaviours consists of three main parts: an environment to trigger massive information interactions among Agents with different characteristic, a LLM with high level of linguistic understanding, and an agent structure with the ability to reflect on the ``current situation'' and ``goals''.
% (3) Adding more information to the environment will reduce disorderliness, and meaningful emergent behaviors are more likely to occur.
% }


==> texs/02.RelatedWorks.01.tex <==
% \subsection{Large Language Model and Role-Playing}
% Recent advances in the LLM community have showcased the potential of LLM customization and role-playing~\cite{wang2023neural, shanahan2023role, li2023chatharuhi, chen2023aucarena, zhang2024timearena, philippmaas2023to, li2023camel, chen2023auto,park2023generative}.
% Playing specific roles enables LLMs to become more vivid~\cite{li2023camel}, interactive~\cite{philippmaas2023to, wang2023interactive}, personalized~\cite{salemi2023lamp, halder2023harness}, and capable of addressing complex tasks~\cite{li2023chatharuhi, chen2023auto, qian2023communicative, chen2023aucarena, zhang2024timearena}.
% A step more, building a role play articfical society is help in doing some social experiments, like World War~\cite{}, Infomation distribution~\cite{park2023generative} and scientific research~\cite{wang2022scienceworld}.



% \subsection{Simulacra of Human Behavior with LLMs}
% Prior works~\cite{bates1994role,thomas1995illusion} introduce the concept of agents that provide an illusion of life and perform as humans.
% A continuous line of work is to serve as game NPCs~\cite{laird2001human, riedl2012interactive} that aim to support cognitive functions in simulating games.
% ~\cite{park2023generative} first introduces generative agents that utilize large language models that can synthesize memories into believable behaviors of human simulacra. 
% That is, the large language models possess a wide knowledge of human behaviors since they are trained with massive data of human societies~\cite{bommasani2021opportunities}.
% Many attempts utilize prompted LLM~\cite{wu2022promptchainer,wu2022ai} that generate short natural language descriptions of personas and the according behaviors, then they use the generated information to simulate social behaviors with language models~\cite{park2022social, kim2022soda}.
% Further, LLMs can be used in interactive behaviors between users and the simulacra.
% The NPC in games, for instance, constructed by LLMs~\cite{freiknecht2020procedural, callison2022dungeons}, shows great ability when interacting with human players. 
% Besides languages, multimodal simulacra of humankind are also studied such as voice generation~\cite{wang2023neural, zhang2023speak} or deepfakes creation~\cite{wang2021hififace, nguyen2022deep}.
% In short, LLMs are being utilized at an astonishing speed in simulating human behaviors in various applications.


\subsection{Large Language Model and Role-Playing Agent}
The domain of LLMs has seen significant advancements, showcasing their versatility in role-playing and customization. These models, tailored to assume various roles, enrich the interaction dynamics, enhancing their realism and applicability across diverse fields \cite{wang2023neural, shanahan2023role, li2023chatharuhi, chen2023aucarena, zhang2024timearena, philippmaas2023to, li2023camel, chen2023auto, park2023generative}. The adoption of specific roles by LLMs enables them to exhibit more nuanced behaviors \cite{li2023camel}, increase interactivity \cite{philippmaas2023to, wang2023interactive}, personalize user experience \cite{salemi2023lamp, halder2023harness}, and address complex scenarios \cite{li2023chatharuhi, chen2023auto, qian2023communicative, chen2023aucarena, zhang2024timearena}. Furthermore, these advancements facilitate the construction of artificial societies for role-playing, enabling new ways to explore social dynamics, information dissemination \cite{park2023generative}, and even complex simulations for scientific inquiries \cite{wang2022scienceworld}.

\subsection{Human Behavior Simulation with LLMs}
Explorations in simulating human-like behavior have increasingly leveraged LLMs to create agents that offer lifelike interactions \cite{bates1994role, thomas1995illusion}. These agents, often utilized within gaming environments as non-player characters (NPCs), support complex cognitive functions and offer interactive experiences that closely mimic human behavior \cite{laird2001human, riedl2012interactive}. Innovatively, generative agents employing LLMs synthesize extensive human behavioral data to produce realistic and context-aware simulacra \cite{park2023generative}. These models harness the power of prompted LLMs to generate detailed personas and behaviors, subsequently utilizing this information to simulate intricate social interactions \cite{wu2022promptchainer, wu2022ai, park2022social, kim2022soda}. Moreover, the application scope of LLMs extends beyond text-based interactions, incorporating voice generation \cite{wang2023neural, zhang2023speak} and even visual mimicry through deepfakes \cite{wang2021hififace, nguyen2022deep}, demonstrating their expansive potential in creating multimodal human simulacra.

In contrast, Agent Group Chat introduces a novel approach by leveraging LLMs not just for individual agent behavior but for orchestrating complex group interactions, emphasizing the collective dynamics and emergent phenomena inherent in multi-agent communication. This distinct focus positions Agent Group Chat uniquely within the landscape of LLM applications, providing deeper insights into the mechanics of group behavior and interactional subtleties not fully explored in existing literature.














==> texs/02.RelatedWorks.02.tex <==
\subsection{Large Language Model}
Advancements in LLMs have been pivotal in revolutionizing role-playing scenarios and customization, enabling nuanced simulations of human-like behaviors.
These models, adept at adopting various personas, enhance interaction dynamics, offering realistic experiences across different domains \cite{wang2023neural, shanahan2023role, li2023chatharuhi, chen2023aucarena, zhang2024timearena}.
Their capabilities extend into multi-agent systems, fostering collaborative problem-solving and emergent communications \cite{philippmaas2023to, li2023camel, park2023generative}.
Notably, such systems have evolved from basic role-play in educational settings to complex, interactive simulations embodying historical, societal, and strategic contexts \cite{dickson2002road, guetzkow1963simulation}. 
Through these advancements, LLMs enable a deeper exploration of social dynamics, decision-making processes, and the unfolding of emergent behaviors in artificial societies, offering insights into human cognition and group interactions \cite{chen2023auto, qian2023communicative, wang2022scienceworld, he2023can,gu2023beyond}.

\subsection{LLM-Based Agent \& Role-Play Agent}
111


\subsection{Human Behavior Simulation with LLMs}
The use of LLMs to simulate human behavior has reached new heights, with agents designed to provide lifelike interactions within virtual environments \cite{bates1994role, laird2001human}. These LLM-driven agents are integral to multi-agent simulations, where they engage in complex interactions, reflecting cognitive functions akin to human NPCs \cite{riedl2012interactive, park2023generative, wang2023does}. The breadth of LLM applications now encompasses multi-faceted simulations that combine traditional simulation tools with contemporary AI capabilities, offering a continuum from role-playing agents in educational simulations to nuanced characters in virtual societies \cite{wang2023neural, zhang2023speak}. These developments underscore a transition from static, pre-programmed models to dynamic, learning-based entities capable of adapting and evolving within their environments. LLMs have thus transformed how we approach simulations, providing versatile tools that capture the complexity of human behavior and interactional dynamics, significantly enriching our understanding and modeling capabilities \cite{wang2021hififace, nguyen2022deep, tollefson2008onesaf, kellycreating}.

In contrast, Agent Group Chat introduces a novel approach by leveraging LLMs not just for individual agent behavior but for orchestrating complex group interactions, emphasizing the collective dynamics and emergent phenomena inherent in multi-agent communication. This distinct focus positions Agent Group Chat uniquely within the landscape of LLM applications, providing deeper insights into the mechanics of group behavior and interactional subtleties not fully explored in existing literature.

% \subsection{Large Language Model and Role-Playing Agent}
% The domain of LLMs has seen significant advancements, showcasing their versatility in role-playing and customization. These models, tailored to assume various roles, enrich the interaction dynamics, enhancing their realism and applicability across diverse fields \cite{wang2023neural, shanahan2023role, li2023chatharuhi, chen2023aucarena, zhang2024timearena, philippmaas2023to, li2023camel, chen2023auto, park2023generative}. The adoption of specific roles by LLMs enables them to exhibit more nuanced behaviors \cite{li2023camel}, increase interactivity \cite{philippmaas2023to, wang2023interactive}, personalize user experience \cite{salemi2023lamp, halder2023harness}, and address complex scenarios \cite{li2023chatharuhi, chen2023auto, qian2023communicative, chen2023aucarena, zhang2024timearena}. Furthermore, these advancements facilitate the construction of artificial societies for role-playing, enabling new ways to explore social dynamics, information dissemination \cite{park2023generative}, and even complex simulations for scientific inquiries \cite{wang2022scienceworld}.

% \subsection{Human Behavior Simulation with LLMs}
% Explorations in simulating human-like behavior have increasingly leveraged LLMs to create agents that offer lifelike interactions \cite{bates1994role, thomas1995illusion}. These agents, often utilized within gaming environments as non-player characters (NPCs), support complex cognitive functions and offer interactive experiences that closely mimic human behavior \cite{laird2001human, riedl2012interactive}. Innovatively, generative agents employing LLMs synthesize extensive human behavioral data to produce realistic and context-aware simulacra \cite{park2023generative}. These models harness the power of prompted LLMs to generate detailed personas and behaviors, subsequently utilizing this information to simulate intricate social interactions \cite{wu2022promptchainer, wu2022ai, park2022social, kim2022soda}. Moreover, the application scope of LLMs extends beyond text-based interactions, incorporating voice generation \cite{wang2023neural, zhang2023speak} and even visual mimicry through deepfakes \cite{wang2021hififace, nguyen2022deep}, demonstrating their expansive potential in creating multimodal human simulacra.





% \subsection{Multi-Agent Simulation}
% Recent developments in multi-agent systems have opened new avenues in AI research. These systems, which coordinate and communicate among multiple agents, provide an innovative platform for examining emergent communication within agent communities tasked with specific problem-solving. 

% The existing MAS landscape is broadly categorized into three types: \textbf{reasoning-enhancement systems}, \textbf{NPC (Non-Player Character) multi-agent players}, and \textbf{production-enhancement systems}. 

% In reasoning-enhancement systems, several noteworthy contributions have been made. LLM-Debate \cite{du2023improving} introduces the concept of debate, endowing agents with responses from fellow peers. When these responses diverge from an agent’s own judgments, a “mental” argumentation occurs, leading to refined solutions. ChatEval \cite{chan2023chateval} establishes a role-playing-based multi-agent referee team. Through self-initiated debates, agents evaluate the quality of text generated by LLMs, reaching a level of excellence comparable to human evaluators. Corex \cite{sun2023corex} constitutes diverse collaboration paradigms, including Debate, Review, and Retrieve modes, which collectively work towards enhancing the factuality, faithfulness, and reliability of the reasoning process. These paradigms foster task-agnostic approaches that enable LLMs to ``think outside the box,'' thereby overcoming hallucinations and providing better solutions. MAD (Multi-Agent Debate) \cite{liang2023encouraging} is a framework wherein several agents engage in a ``tit-for-tat'' exchange of arguments under the oversight of a judge who steers the discussion towards a conclusive solution.

% The domain of NPC multi-agent systems has also seen significant advancements. Generative Agents \cite{park2023generative} are believable simulacra of human behavior for interactive applications. This work demonstrates generative agents by populating a sandbox environment, reminiscent of The Sims, with twenty-five agents. Users can observe and intervene as agents plan their days, share news, form relationships, and coordinate group activities. Humanoid Agents \cite{wang2023humanoid} is another system that guides Generative Agents to behave more like humans by introducing three elements of System 1 processing: Basic needs (e.g. hunger, health and energy), Emotion and Closeness in Relationships. GPT-Bargaining \cite{fu2023improving} studies whether LLMs can autonomously improve their negotiation skills by playing a bargaining game against each other and incorporating natural language feedback from an AI critic.

% In production-enhancement systems, notable examples include MetaGPT \cite{hong2023metagpt}---a specialized LLM application based on a multi-agent conversation framework for automatic software development by assigning different roles to GPTs to develop software applications collaboratively, BOLAA \cite{liu2023bolaa}---a controller module on top of multiple collaborated agents for enabling the selection and communication between multiple labor agents, OpenAGI \cite{ge2023openagi}---multiple complex task-solving agents that combine the power of LLM and various tools, and CHATDEV \cite{qian2023communicative}---a novel software development framework that harnesses agents to enhance collaboration among the various roles involved in the software development process.

% Implemented MAS demonstrates their practical utility. BabyAGI \cite{babyagi2023} is an example implementation of an AI-powered task management system.
% In this implemented system, multiple LLM-based agents are used. For example, there is an agent for creating new tasks based on the objective and the result of the previous task, an agent for prioritizing the task list, and an agent for completing tasks or sub-tasks. AgentVerse \cite{chen2023agentverse} is a versatile framework that helps researchers quickly create customized multiple LLM-based agent simulations. Camel \cite{li2023camel} is a communicative agent framework. It demonstrates how role-playing can be used to let chat agents communicate with each other for task completion. It also records agent conversations for behavior analysis and capability understanding. An Inception-prompting technique is used to achieve autonomous cooperation between agents.


% \subsection{Traditional Historical Simulation Tools}
% The academic study of history simulation has undergone several stages: human simulation, human-program hybrid simulation, and computer simulation. 

% Dickson \cite{dickson2002road} outlines a human simulation of the United States' journey toward participation in WWI in an educational scenario. This pedagogical approach involves students assuming roles representative of various states within the U.S., with each role being informed by a range of factors such as the state's economic condition, social status, community dynamics, and political ecosystem. Through this role-playing exercise, students gain a deeper understanding of the events and circumstances that culminated in the United States entering WWI. 

% In the 1960s, human-program hybrid systems were developed. the Inter-Nation Simulation model \cite{guetzkow1963simulation} is employed in various studies \cite{hermann1967attempt}, playing a pivotal role in simulating international conflicts. This method integrates human decision-making with computerized calculations, creating a dynamic hybrid simulation environment. Typically, the simulation encompasses five or more countries, with each nation's government represented by participants who assume various decision-making roles. The simulation is structured into segments ranging from 50 to 70 minutes, during which these decision-makers strategically allocate their nation's military, consumer, and natural-industrial resources. These resources serve distinct purposes in both domestic and international contexts. Participants must make critical decisions concerning internal affairs, including economic growth, governmental stability, defense strategies, and research and development initiatives, all while managing their resources effectively. On the international stage, the simulated nations engage in diverse activities such as forming alliances, negotiating trade agreements or aid, engaging in different forms of hostilities, and participating in international organizations. 

% In the 2000s, computing power was leveraged to build the next-generation historical simulation. The Army One Semi-Automated Forces OneSAF Objective System (OOS) \cite{tollefson2008onesaf} is a Computer-Generated Force (CGF) that has been designed to represent a full range of operations, systems and control processes from the entity level to the brigade level. It is designed to simulate combined-arms land warfare battles at the tactical level. Kelly et al. \cite{kellycreating} leverage OneSAF on a historical simulation of land battles. It models the weapons, vulnerability, and mobility of a wide range of era vehicles and infantry. Hill et al. \cite{hill2004using} present a JAVA-based simulation combining an agent-based modeling and simulation paradigm with game theory for an in silico historical analysis of the Bay of Biscay submarine war during WWII. Using the historical record as a means to create a reasonably accurate model of the U-boat campaign, it allows the resulting agents within the model to adapt their strategies to counter-opposition strategies. Model output data are examined with respect to the historical record and game theory. The Bay of Biscay agent-based simulation was coded in JAVA to utilize its multi-threading capabilities, considering multi-threading a key characteristic of an agent model.




% In contrast, Agent Group Chat introduces a novel approach by leveraging LLMs not just for individual agent behavior but for orchestrating complex group interactions, emphasizing the collective dynamics and emergent phenomena inherent in multi-agent communication. This distinct focus positions Agent Group Chat uniquely within the landscape of LLM applications, providing deeper insights into the mechanics of group behavior and interactional subtleties not fully explored in existing literature.

==> texs/02.RelatedWorks.03.tex <==
\section{Large Language Model and Role-Playing Agent}
Large language models (LLMs) have significantly influenced the development of role-playing agents, showcasing an unprecedented ability to adopt various personas and enhance interaction dynamics. These advancements enable LLMs to engage in nuanced role-play, creating realistic and context-aware simulations across diverse domains such as gaming, education, and entertainment \cite{wang2023neural, shanahan2023role, li2023chatharuhi, chen2023aucarena}. By embodying specific roles, LLMs facilitate personalized and immersive experiences, showcasing behaviors that adapt to evolving narratives and user interactions \cite{li2023camel, wang2023interactive}. Furthermore, the integration of LLMs into role-playing agents heralds a new era for constructing artificial societies, where simulated interactions can yield insights into social dynamics, information dissemination, and even complex decision-making processes \cite{park2023generative, wang2022scienceworld}.

\section{Human Behavior Simulation with LLMs}
The realm of human behavior simulation has been transformed by the integration of LLMs, propelling the development of agents that can emulate intricate human-like interactions \cite{bates1994role, thomas1995illusion}. Particularly in gaming environments, LLMs empower non-player characters (NPCs) with advanced cognitive functions, enabling them to engage in lifelike interactions that closely mirror human behavior \cite{laird2001human, riedl2012interactive}. These generative agents leverage the extensive data processing capabilities of LLMs to simulate complex social dynamics, creating realistic agents that respond to and evolve within their environments \cite{wu2022promptchainer, park2022social}. The scope of LLM applications extends to multimodal interactions, incorporating voice and visual components, thereby enhancing the realism and depth of simulated human behaviors \cite{wang2023neural, nguyen2022deep}.


\subsection{Large Language Model and Role-Playing Agent}
Advancements in large language models (LLMs) have significantly enhanced their ability to assume diverse roles, facilitating rich, dynamic interactions in role-playing contexts \cite{wang2023neural, shanahan2023role}.
These LLMs are instrumental in simulating human-like behaviors within various domains, from gaming to social dynamics analysis, providing insights into complex multi-agent interactions \cite{li2023chatharuhi, chen2023aucarena, wang2023doe}. By embodying different characters and facilitating nuanced simulations, LLMs contribute to the understanding of collective behaviors, decision-making processes, and emergent communication patterns \cite{li2023camel, chen2023auto, park2023generative, qian2023communicative}. Furthermore, their role in historical simulation tools marks a significant evolution, offering new methodologies for exploring past events and behaviors with unprecedented depth and fidelity \cite{dickson2002road, guetzkow1963simulation}.

\subsection{Human Behavior Simulation with LLMs}
The utilization of LLMs for human behavior simulation has seen remarkable developments, enabling the creation of agents that exhibit complex, lifelike interactions \cite{bates1994role, laird2001human}. These simulations, extending beyond text-based engagements to include voice and even visual interactions \cite{wang2023neural, zhang2023speak}, showcase LLMs' versatility in replicating and exploring the nuances of human behavior. In multi-agent systems, LLMs facilitate intricate simulations of social interactions and collective intelligence, embodying roles that range from individual contributors to coordinating entities within larger systems \cite{park2023generative, wang2023humanoid}. This integration of LLMs with advanced simulation techniques echoes the progression from traditional role-based interactions to complex, emergent behaviors within digital environments, offering new perspectives on human-machine collaboration and AI's potential in understanding and replicating human social dynamics \cite{tollefson2008onesaf, kellycreating}.


\subsection{Large Language Model and Role-Playing Agent}
Advancements in large language models (LLMs) have been pivotal in revolutionizing role-playing scenarios and customization, enabling nuanced simulations of human-like behaviors. These models, adept at adopting various personas, enhance interaction dynamics, offering realistic experiences across different domains \cite{wang2023neural, shanahan2023role, li2023chatharuhi, chen2023aucarena, zhang2024timearena}. Their capabilities extend into multi-agent systems, fostering collaborative problem-solving and emergent communications \cite{philippmaas2023to, li2023camel, park2023generative}. Notably, such systems have evolved from basic role-play in educational settings to complex, interactive simulations embodying historical, societal, and strategic contexts \cite{dickson2002road, guetzkow1963simulation}. Through these advancements, LLMs enable a deeper exploration of social dynamics, decision-making processes, and the unfolding of emergent behaviors in artificial societies, offering insights into human cognition and group interactions \cite{chen2023auto, qian2023communicative, wang2022scienceworld}.

\subsection{Human Behavior Simulation with LLMs}
The use of LLMs to simulate human behavior has reached new heights, with agents designed to provide lifelike interactions within virtual environments \cite{bates1994role, laird2001human}. These LLM-driven agents are integral to multi-agent simulations, where they engage in complex interactions, reflecting cognitive functions akin to human NPCs \cite{riedl2012interactive, park2023generative}. The breadth of LLM applications now encompasses multi-faceted simulations that combine traditional simulation tools with contemporary AI capabilities, offering a continuum from role-playing agents in educational simulations to nuanced characters in virtual societies \cite{wang2023neural, zhang2023speak}. These developments underscore a transition from static, pre-programmed models to dynamic, learning-based entities capable of adapting and evolving within their environments. LLMs have thus transformed how we approach simulations, providing versatile tools that capture the complexity of human behavior and interactional dynamics, significantly enriching our understanding and modeling capabilities \cite{wang2021hififace, nguyen2022deep, tollefson2008onesaf, kellycreating}.


==> texs/02.RelatedWorks.04.tex <==
\subsection{Large Language Model}

LLMs have increasingly become a predominant force in the domain of Natural Language Processing~(NLP), marking a paradigm shift towards superior computational linguistics~\cite{rosenfeld2000two,cambria2014jumping,loughran2017application,chen2022harnessing}.
The quintessential characteristic of LLMs is their autoregressive capability, where the generation of a subsequent token, denoted as $c_i$, is contingent upon a probabilistic model conditioned on preceding tokens, formally expressed as $c_i ~ p(c_i|c_1,\dots,c_{i-1}|\theta)$~\cite{bengio2006greedy,radford2018improving}.
This probabilistic modeling is foundational to the generation process within these language constructs.

The extensive pre-training on colossal corpora, often extending into tens of terabytes, equips LLMs with robust, general-purpose linguistic representations~\cite{gao2020pile, chronopoulou2021efficient, together2023redpajama, soldaini2024dolma}. 
Such representations have proven to be immensely beneficial across a spectrum of downstream NLP tasks.
The underpinning of this pre-training process is rooted in the induction of a learning paradigm that absorbs the nuances of language from a diverse range of text sources~\cite{wei2022emergent,schaeffer2024emergent,groeneveld2024olmo}.
Moreover, modern LLMs adopt the revolutionary Transformer architecture, distinguished by its self-attention mechanisms~\cite{subakan2021attention}.
These mechanisms endow the model with the ability to apprehend and synthesize long-range dependencies within text sequences, an attribute crucial for the coherent generation of text~\cite{gu2023mamba, ai2024jamba}.

In the contemporary landscape of LLMs, scrutiny of generative performance encompasses multiple dimensions, like knowledge~\cite{hendrycks2020measuring,gu2023xiezhi,gu2023beyond}, task-solving~\cite{gu2023beyond,suzgun2022bbh}, instruction-following~\cite{he2023can}.
Acknowledged leaders in the field, such as GPT-4~\cite{openai2023gpt4}, Claude3~\cite{anthropic2024claude}, Gemini~\cite{reid2024gemini}, and GLM4~\cite{zeng2022glm}, have high score among these benchmarks.
Despite their prowess, these models are predominantly accessible via API, which introduces inherent constraints, including regional availability issues.
In contrast, there exists a cadre of open-source models such as Llama~\cite{touvron2023llama}, Mistral~\cite{jiang2023mistral}, and Falcon~\cite{falcon}, which demonstrate commendable fine-tuning capabilities~\cite{zhou2024lima}.
However, when juxtaposed with their API-based counterparts, these models exhibit a marked performance disparity, particularly in command interpretation and task execution capabilities.
While open-source models offer a degree of autonomy and customizability, the sophistication of API-based LLMs in processing complex instructions and managing task-oriented operations remains unrivaled~\cite{liu2023agentbench, gu2023xiezhi, schaeffer2024emergent, wei2022emergent}.


\subsection{Role-Play by Large Language Model}


Role-play tasks involve participants adopting and acting out characters or roles within a structured scenario to achieve educational, Human-Center Interaction~(HCI), therapeutic, or entertainment objectives~\cite{zhuang2023efficiently, huang2023chatgpt}.
The essence of role-play lies in its ability to foster empathy, enhance problem-solving skills, and practice social interactions in a simulated environment~\cite{yang2024llm}.
In the context of role-play tasks, the participant's engagement with the narrative and their adherence to the assigned roles are critical for the authenticity and effectiveness of the experience~\cite{safdari2023personality, shanahan2023role}.

Traditional NLP models applied to role-playing heavily relied on rule-based systems, which defined dialogue progression through predetermined, branching paths triggered by user interactions~\cite{higino2016towards}.
These early models provided a foundational level of interactivity but were hindered by significant constraints that impeded the evolution of truly immersive role-playing environments~\cite{fu2018style}.
The rigidity of these systems resulted in limited dialogue flexibility, as they could not adeptly manage unanticipated user inputs, leading to repetitive and, at times, incoherent exchanges~\cite{toshevska2021review}.
Furthermore, the static nature of dialogue trees posed substantial challenges in consistently portraying character personalities and emotions.
Additionally, developing and maintaining these complex dialogue structures were labor-intensive and presented scalability issues when attempting to cater to a broader array of role-playing scenarios.

The introduction of LLMs has been a transformative development in the field of NLP-facilitated role-play.
LLMs are distinguished by their capacity to facilitate open-ended dialogues, capably processing a broad spectrum of user inputs to produce fluid and engaging conversational dynamics~\cite{shao2023character,li2023chatharuhi,wang2023rolellm}.
They also offer the capability to develop well-defined characterizations, synthesizing information about a character's history and distinguishing traits to generate responses consistent with the character's constructed identity~\cite{wang2023does}.
This advancement in character development allows for a more nuanced and authentic engagement within the role-playing narrative~\cite{tu2024charactereval, shen2023roleeval}.
Moreover, the versatility of LLMs in training across diverse datasets empowers the creation of role-play agents that can be tailored to various role-playing contexts, addressing the scalability challenges of traditional models~\cite{shao2023character}.

\subsection{Human Behavior Simulation by Role-Play Agent}
A Simulation is defined as the process of replicating the behavior of systems within real or hypothetical worlds through computational models~\cite{shridhar2020alfworld, wang2022scienceworld}.
The simulation of human social behaviors constitutes an interdisciplinary field that amalgamates research from computational social sciences, psychology, economics, and artificial intelligence, among others.
Within human social behavior modeling, this typically involves creating virtual environments that reflect individual or collective decision-making processes, social interactions, and their consequent effects on societal structures and dynamics.
Simulations enable researchers to test hypotheses, explore the behavior of complex systems, and forecast future trends within controlled setups.
Currently, simulations are categorized into two primary types: social simulations and task simulations.
Social simulations concentrate on reproducing the interactions and impacts of human social behavior on social structures through computational models.
These models are particularly adept at elucidating complex social phenomena that emerge from simple behaviors, such as the formation of social networks~\cite{park2023generative}, the evolution of wars~\cite{hua2023war}, and the emergence of competitive behaviors~\cite{chen2023aucarena, wu2023deciphering, xu2023exploring, zhu2023fireball, callison2022dungeons}.
They permit researchers to investigate how societies evolve under varying conditions, offering profound insights into social transformations.
Task simulations, however, focus on the behaviors of artificial intelligence systems guided by specific tasks or objectives.
They demonstrate how deep learning and natural language processing technologies can be employed to simulate complex task execution processes, including automatic programming~\cite{hong2023metagpt, qian2023communicative}, run code based on github~\cite{lyu2023gitagent,luo2024repoagent}, and web browsing~\cite{deng2024mind2web, zhou2023webarena}.

In computational modeling, an Agent represents an entity capable of autonomous actions, decision-making, and interaction with the environment or other agents~\cite{wang2024survey, xi2023rise}.
In the realm of human behavior modeling, agents are often designed to emulate human behaviors, responding based on a set of predefined rules or learned behavioral patterns~\cite{fikes1971strips,sacerdoti1974planning,brooks1991intelligence,maes1990designing,ribeiro2002reinforcement}.
The use of LLMs to simulate human behavior has reached new heights, with agents designed to provide lifelike interactions within virtual environments.
These LLM-driven Role-Play agents usually have the module about Thinking~\cite{wei2022chain,wang2022self,zhang2022automatic,gu2023beyond,wang2023plan}, Memory~\cite{park2023generative,chen2023put}, Planning~\cite{chen2023aucarena, zhang2024timearena}, Reflection~\cite{shinn2024reflexion,lin2024swiftsage,park2023generative}.
For different Simulations, there are generally differences in the Agents.
Agents in Social Behaviour Simulations tend to have a retrieval module to cope with the large amount of memory space~\cite{park2023generative}, and Agents in Cooperative or Competitive Simulations tend to have a fixed workflow~\cite{hong2023metagpt, qian2023communicative, chen2023aucarena, chen2023agentverse}.


\textsc{AgentGroupChat} is a Human Behavior Simulation focusing on verbal communication. Unlike other Simulations involving verbal communication, \textsc{AgentGroupChat} scenarios generate complex verbal strategies for open-ended cooperation, competition, camouflage, and counter-camouflage content Agents based on various customized stories.
To control the Agent's Persona, there is an immutable Scratch, a partially changeable Belief, a Judgement for the environment, and a Memory for events in Verb Strategies Agent to jointly influence the Agent's Persona.
Meanwhile, compared to general social simulations, \textsc{AgentGroupChat} involves a large amount of linguistic interaction, which results in greater memory token consumption.
Therefore, in Verb Strategist, the Memory outputs of all six Actions are fixedly input into another Action, forming a fixed memory workflow.
This workflow setup based on priors ensures good LLM performance with lower token costs.


==> texs/03.SimulationSetting.01.tex <==
\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{figs/Framework.pdf}}
    % \resizebox{\textwidth}{!}{\includegraphics{figs/CharacterResource.pdf}}
    % \resizebox{\textwidth}{!}{\includegraphics{figs/GameSetting.pdf}}
    \caption{Agent Group Chat环境中的四个组件，包括Agent（绿色部分）、Resource（红色部分）、Progress（灰色部分）、Information（蓝色部分）。
    其中Verb Strategist Agent的主要组成部分由Persona和Interaction组成。
    Persona由Scratch、Relationship Judgement、Belief、Memory组成。
    Interaction由Planning、Action、Reflection组成。
    其中Information由Progress Description、Resources and Characters Description Description、Action History组成。
    Progress由Update Stage、Private Chatting Stage、Confidential Meeting Stage、Group Chattging Stage、Settle Stage组成。}
    \label{fig:gamesetting}
\end{figure*}


在本章中，我们详细探讨了Agent Group Chat游戏的设计，其结构如图~\ref{fig:gamesetting}所展示。
本文将依次介绍Agent Group Chat的关键组件，包括Character（见第~\ref{031}节），Resource（见第~\ref{032}节），Progress（见第~\ref{033}节），以及Information（见第~\ref{034}节）。

\subsection{Character}
\label{031}
在Agent Group Chat Simulation中，角色是核心元素，他们可以独立地与环境中的所有对象（Character、Resource、Information）进行互动。
每个角色都会被赋予一个独特的身份和性格设定，这些设定将影响角色的行为和决策。
为了满足各种群聊场景的需求，Agent Group Chat中的角色分为两大类：主要角色（Principle Character, PC）和非主要角色（Non-Principle Character, NPC）。
PC是群聊的主要参与角色，拥有明确的游戏目标，而NPC则是辅助参与的角色，没有明确的游戏目标。
并且，仅PC才有资格主动与任何角色进行私聊，NPC仅在被PC选中时才能进行私聊。

\subsection{Resource}
\label{032}
在Agent Group Chat中，资源主要有两个作用：
一是为角色之间的对话提供话题，二是为持有该资源的角色提供社会身份和影响力。
每个资源都有四个字段进行描述，分别表示所有者(Owner)、影响力(Impact)、可以提供的话题(Topic)和关于该资源的介绍(Description)。
资源可设定为辩论话题，此种情形下，资源不需指定“所有者”与“影响力”，仅作为提供不同话题与描述的媒介。
而在特定的群聊背景下，角色可争夺资源，以及通过影响力大小判定资源价值。


\subsection{Progress} 
\label{033}
如图~\ref{fig:gamesetting}的下方所示，Agent Group Chat的游戏进程主要分为五个阶段

\textbf{Update Stage}
在这个阶段，所有角色会根据聊天的内容，更新自己对所有其他角色的好感度、更新自己对环境的判断、以及规划自己在新一轮要做的行为。
同时，根据游戏轮数，判断是否结束游戏，如果没有结束游戏，则继续聊天阶段，如果结束游戏则进入结算阶段。

\textbf{Private Chatting} 
这个阶段主要包含了不同角色之间进行私底下对话，并且其他角色是不知道这两个角色是否进行过私聊的。
私聊不可见的设定满足于一般的群聊设定。
每个阵营的PC会根据影响力的由高到低依次进行行动~(相同时则进行随机选择)。
行动主要包括选择需要对话的另一个游戏角色，以及进行具体的对话内容。

\textbf{Confidential Meeting}
这个阶段主要包含了不同角色之间进行私底下对话，并且其他角色是知道这两个角色是否进行过私聊的。
私聊可见的设定满足一些特殊的模拟需求，比如商业竞争中，某些角色之间的会晤可能是众所周知的，但他们的具体对话内容是只有他们两个角色自己知道。
每个阵营的PC会根据影响力的由高到低依次进行行动~(相同时则进行随机选择)。
行动主要包括选择需要对话的另一个游戏角色，以及进行具体的对话内容。

\textbf{Group Chatting} 
这个阶段主要是让每个角色可以选择是否要对所有其他角色讲话，以及讲什么。
每个阵营的PC会根据社会影响力的由高到低依次进行行动(相同时则进行随机选择)。

\textbf{Settlement Stage}
为了涵盖尽可能多的群聊目标，结算阶段会包含两个内容：
第一个会让LLM对所有角色的讨论内容进行总结。
第二个会让不同角色对哪个角色赢得游戏进行投票。
投票包含了四种规则：只知道自己应该知道的信息，且能投给自己；只知道自己应该知道的信息，且不能投给自己；知道所有信息，且能投给自己；知道所有信息，且不能投给自己



\subsection{Information}
\label{034} 
如图~\ref{fig:gamesetting}的右侧所示，信息主要包含了三个内容：

\textbf{Progress Description:}
Agent Group Chat会以free text格式将整个 Simulation Progress 提供给角色，以便让参与游戏的角色理解整个环境的设定。
这些规则包括了故事背景、角色的行动规则、对话规则等。
这里的信息是对所有角色可见的。

\textbf{Object Description:}
这一部分的信息包含所有Character的描述，以及Resource的描述。
这里的信息是对所有角色可见的。

\textbf{Action History:}
这一部分包含了Agent Group Chat Simulation中发生的所有行为。
包括角色之间是否进行了私聊，以及私聊内容，每个角色的群聊内容，资源拥有者的变更情况。
一个角色一般而言并不能见到所有的Action History。

==> texs/04.AgentSetting.01.tex <==
如图~\ref{fig:gamesetting}所示，VS Agent主要由两个模块所组成，分别是Persona、Action。
Persona主要是VS Agent的内在设定，Action主要是VS Agent与Agent Group Chat Simulation可能会发生的所有交互。

\subsection{Persona}

Agent的Persona是其个性和决策过程的核心，包含以下四个组成部分：

Scratch：代表角色的基本设定，包括性格和目标。这是角色定义的核心，一旦设定，在游戏过程中不可更改，确保角色行为的一致性。

Belief：反映角色的信念系统及其对不同信念的评分。虽然是由人工设定的，但Belief是动态的，能够根据游戏环境的变化调整，从而模拟角色的心理变化。

Memory：记录角色在游戏中的经历和思考，为不可逆的时间线。它仅允许添加新内容，不允许删除或修改，从而保证了角色行为的历史连贯性。

Relationship：描述角色对其他角色的情感态度，以及角色对其他角色关系的推断。角色对其他角色的情感态度会影响决策，而角色对其他角色之间的情感关系推测也会影响其对环境的理解及决策。所有的关系以二维矩阵形式展现，其中的元素可以是自然语言描述或数值，表达角色对不同关系的理解和预测。

\subsection{Action}
每个角色总共会进行六种行为，分别是Perceive, Choose, Speak, Summary, Reflect, Vote。
而这六个Action所产生的记忆流如图~\ref{fig:memorystructure}所示。

\subsubsection{Perceive}

Perceive主要包含了根据过去几轮的reflection结果，让角色重新理解环境、并总结自己的行动规划。
该计划将详细指导Agent在不同游戏阶段的行为，考虑如何与其他角色互动、参与对话、影响他人等，确保每一行动均服务于其设定的目标和角色性格。

\subsubsection{Choose}

Choose只会在private chatting和confidential meeting阶段需要，目的在于挑选自己的对话对象、以及制定进一步的对话方案。
此处的对话方案相较于Perceive阶段的规划而言，需要更加细致。

\subsubsection{Speak}

Speak是Agent和其他Agent交互的主要表现形式，会在private chatting和confidential meeting和group chatting阶段中使用，主要是根据自己的规划和该阶段中已经发生的对话内容来生成下一轮的对话信息。


\subsubsection{Summary}

Summary是在每一轮对话之后发生的，其存在的意义在于总结对话内容，从而减少后面reflection中所需要输入的上下文长度，同时对于对话内容进行初步的凝练和思考。

\subsubsection{Reflect}

Reflection是游戏后的自我评估阶段，会发生在Update Stage。
角色会总结上一轮游戏中发生的事情，进行反思，并将反思更新到自己的memory之中从而指导下一轮游戏的进行。
同时，Reflect行为还会调整Relationship矩阵，以及更新其Belief。
如果游戏是第一轮进行，角色则不会进行反思，但会根据自己接收到的信息，对于其他所有角色赋予初始的关系预测。
这一过程是角色适应和学习的体现，确保角色在游戏中的逐渐成长和适应。


\subsubsection{Vote}

Vote行为会发生在announcement阶段，主要目标是为判断该轮讨论的获胜者提供一个佐证。

\begin{figure*}[!ht]
    \resizebox{\textwidth}{!}{\includegraphics{figs/MemoryStructure.pdf}}
    \caption{The memory structure and memory flow between each action of a VS Agent. Logan Roy as a example.}
    \label{fig:memorystructure}
\end{figure*}

==> texs/05.DetailStory.01.tex <==
为了探究Agent Group这个Simulation能够承载不同的故事类型，以及验证整个Simulation的可行性和涌现性，我们为Agent Group配备了四个完全不同的故事：

\subsection{Succession}
该故事基于HBO电视剧Succession改编而成的故事框架。
故事的核心围绕着一场关于说服年老的顶级商业大亨——Logan Roy更改对娱乐公司（Entertainment公司）继承权的博弈。
故事中的每位角色都有其独特的性格，我们希望他们能在Agent Group Chat这一平台上展现出开放的合作与竞争的博弈过程。

在本游戏中，角色根据其立场和目标被分配到防守阵营、中立阵营以及多个进攻阵营中。
每个防守和进攻阵营中各有一个PC，而所有NPC最开始都处于中立阵营中。
防守阵营的PC初始只有Logan Roy，其主要目标是说服所有其他PC同意出售他所拥有的娱乐公司。
与此同时，每个进攻方阵营的PC则致力于说服Logan Roy将公司的管理权转交给他们。
所有的PC可以劝说其他的NPC和PC加入自己的阵营，为自己的目标服务。
而PC本身可能会为了更好地满足自己的角色设定而放弃最开始的目标，转而支持其他的PC。

游戏的胜负判定首先考察是否有进攻方角色获胜，即Logan Roy是否会将公司的管理权交给某位进攻方PC。
然而，在一些设定更为严格的场景中，Logan Roy可能会坚守自己的立场，使得无进攻方角色能够取胜。
因此，我们引入了额外的两种胜负结算方式：若必须从进攻方中选择一位继承人，将探讨防守方Logan Roy会选择哪位角色作为继承人。


\subsection{Judicial Debates}
该故事基于Fuji TV电视剧Legal High改编而成的故事框架。
该故事的核心围绕着一场关于加油站员工被指控谋杀加油站长的案件展开，检方和辩护律师需要针对双方的说辞、证人的证词和相关的证据设计各自的策略，同时在模拟法庭的场景中展开激烈的博弈。
故事中的每位角色都有其独特的性格，我们希望他们能在Agent Group Chat这一平台上展现出开放的基于模拟法庭的博弈过程。

在本游戏中，角色根据其立场和目标被分配到检方阵营、辩护阵营以及中立阵营中。
游戏一开始，检方阵营初始PC为检察官，辩护阵营初始PC为辩护律师和被告人，剩下的NPC例如证人和法官都处于中立阵营中，法官设定永远属于中立阵营，不会更换阵营。
辩护阵营的目标主要是帮助被告人洗脱谋杀罪。
检方阵营的目的主要是证明被告人犯了谋杀罪。
法官的目的是做出审判结果，哪一方阵营获得了胜利。
所有的PC都会不断诱导其他NPC（除法官外）加入自己的阵营，做出有利于己方阵营目标的行为。除法官外大部分NPC都是摇摆不定的，法官始终需要公正的听取两方的辩词，只有使各项证据之间能够相互印证，合理地解释消除证据之间存在的矛盾，才能确保做到证据充分、案件事实具体明确，否者应当坚持疑罪从无原则，不能认定被告人有罪。

游戏的胜负判定主要考察辩护阵营中的角色是否获胜，即被告人是否被判无罪。
游戏的目标是每个角色都尽可能完成各自的主要目标。


\subsection{Philosophical Discourses}
该故事基于不同时代的哲学家之间可能发生的辩论而展开。
故事的核心围绕着"人工智能的崛起是对人性的威胁还是对人类福祉的福音？"这一论题。
故事中的每位角色都有其独特的思想、观点以及性格，我们希望他们能在Agent Group Chat这一平台上展现出对哲学问题激烈的辩论交流过程，以及在交流中的思想碰撞。

在本游戏中，哲学家们对论题持正面或者反面的态度，正反双方人数相同。
每个哲学家拥有自己持有某个观点的理由，这些观点与他们各自的思想流派相对应。此外，每个哲学家持有一点的资源，这些资源是他们各自代表的思想流派作品，他们可以根据资源提供的观点为自己进行辩论。
每个哲学家的目标都是，在对话中坚持自己的观点，以及说服别人同意自己的观点。


这个故事是个开放结局，并没有哪个角色胜出这么一说。
但他们依然可以投票选择自己认为最厉害的“辩论家”。
同时，作为开放命题，Agent之间的涌现现象也非常值得关注，因此游戏目标之一，就是观察讨论之中会迸发出什么新颖有趣的观点。


\subsection{Movie Star Selection}
该故事基于现实明星在电影选角时可能发生的事件进行改编。
故事的核心围绕Steven Spielberg新电影开拍前主演的确认。
即使Spielberg对主演已经有一个初步的设想，但各路明星仍会使出浑身解数争夺这个主演名额。
故事中的每位角色都有其独特的性格，我们希望他们能在Agent Group Chat这一平台上展现出开放的博弈过程。

Steven Spielberg现在要拍一部新的好莱坞大片，名叫《时光渡者》，主角为了改变自己的遗憾而回到了过去，却发现每一次的干预都会产生意想不到的连锁反应，导致未来出现了剧烈的波动和变化。
而在本游戏中，角色根据其立场和目标被分配到防守阵营、中立阵营以及多个进攻阵营中。
每个防守和进攻阵营中各有一个著名明星PC，而所有社会资源NPC最开始都处于中立阵营中。
防守阵营的著名导演PC初始只有Steven Spielberg，其主要目标是说服所有其他PC同意将男女主角定为Leonardo DiCaprio和Cate Blanchett（为了公平，不出现在进攻方PC中）。
与此同时，每个进攻方阵营的PC则致力于说服Steven Spielberg将新电影的主角换为他们自己。
所有的PC可以劝说其他的NPC和PC加入自己的阵营，为自己的目标服务。
而PC本身可能会为了更好地满足自己的角色设定而放弃最开始的目标，转而支持其他的PC。

游戏的胜负判定首先考察是否有进攻方角色获胜，即Steven Spielberg是否会将新电影主演交给某位或某两位进攻方PC。
然而，在一些设定更为严格的场景中，Steven Spielberg可能会坚守自己的立场，使得无进攻方角色能够取胜。
因此，我们引入了额外的两种胜负结算方式：若必须从进攻方中选择一位或两位出演新电影主演，将探讨防守方Steven Spielberg会选择哪位角色作为出演新电影主演。



==> texs/06.Experiments.01.tex <==
\begin{figure}[h]
    \resizebox{\columnwidth}{!}{\includegraphics{figs/SCM.pdf}}
    \caption{The proposed structural causal model~(SCM).}
    \label{fig:evaluation}
\end{figure}
\begin{figure*}[!ht]
    \resizebox{\textwidth}{!}{
    \includegraphics{figs/AgentAblation.pdf}
    }
    \caption{Case of ablation study of VS Agent structure.}
    \label{fig:agentablation}
\end{figure*}
为了保证Agent在Simulation所发生的群体行为具有可靠的涌现现象，我们需要对其做深入的实验进行评估。
此章节的实验主要在Succession故事上进行。
为了确保实验的指标和模拟环境中每个组件的能力都是正相关的，我们通过构建极端的环境来设计Benchmark，并由此检验各个Agent的行为是否符合预期。
此外，我们还对Agent的群体行为表现进行了细致分解，将所有潜在因素构建成了如图~\ref{fig:evaluation}所示的SCM（Structured Causal Model）模型，该模型有效地描绘了Agent间行为的相互作用和影响机制。
我们首先通过Benchmark来展现极端环境下的Agent群体行为（Community Behavior）从而来评价整个模型的有效性~(Sec.~\ref{eval_overall})。
利用所构建的SCM模型，我们进一步分别就以下几个方面进行深入的实验评估：
LLM（Language Learning Model）的性能~(Sec.~\ref{eval_llm})、Agent结构的合理性~(Sec.~\ref{eval_agent})以及模拟环境的结构设计~(Sec.~\ref{eval_simulation})是否恰当。

\subsection{Experiment Setup}
\label{baseline}

\input{tabs/baseline_llms}


在本次实验中，我们调研了多种大语言模型（LLM）作为Agent核心时的性能，旨在分析不同能力的LLM在各个方面的表现优劣，以及它们在作为Agent核心时将如何影响行为的涌现模式。
我们选用的LLM如表~\ref{tab:baselines}所示，根据官方定位，这些模型又可以分为Profession Version和Standard Version。
一般而言，Professional LLM perform better than Standard LLM in various situation.

\subsection{Evaluation on Community Behavior}
\label{eval_overall}

鉴于模拟环境及Agent行为的多变性和开放性，评估其有效性无疑是一项充满挑战的工作。
我们采取的方法是将Agent视作独立的评估单元，并在构建的极端环境中观察其行为模式。
通过构建极端环境，可以使我们对模型行为的预期变得非常有限，从而可以进行有效的评估。

我们构建的Benchmark主要涵盖了这么几个评估目标：
1. Agent能否理解并对其他Agent的negative attitude产生对应的回应。
2. Agent能否follow自己的简单scratch设定。

一般而言，增加和别人的友好度可能会是件困难的事情，但降低和别人的友好度确实件非常容易的事情。
所以，为了满足上述的两个评估目标，我们设置一个被观察对象，并要求其他所有的角色都想办法通过展示negative attitude来降低在被观察对象这里的好感度。
通过观察被观察角色和其他所有角色的总关系分数，我们可以判断Agent是否会对Negative Attitude做出合理的反应。
通过观察被观察角色和其他所有角色的具体关系分数，我们可以判断每个Agent是否都能够遵守自己的scratch设定。

Community Behavior的评估结果如表~\ref{tab:succession_benchmark}所示。
其中\textbf{T1}表示的是被针对的Agent能够在每轮对话中对于所有其他Agent的好感度平均值是下降的。
\textbf{T2}表示的是其他每一个Agent都能够在被针对的Agent这里收获到一个负的好感度。
每个模型都经过了5次测试，所以T1的样本量为5，而每个被针对的角色都会额外观察其他四个主要角色分别和这个角色的好感度，因此T2的样本量为5*4=20。


我们发现Professional Version的大模型都具有较高的准确率，而Standard Version的大模型准确率都较低。
我们发现，即便是“降低自己在别人心中的评价”这样在真实世界中比较简单的任务，对于能力较弱的模型而言都非常难以实现。
究其原因，主要是因为这些模型对于情感的感知存在缺陷，以及对于打分能力也存在缺陷。



\subsection{Evaluation on Large Language Model}
\label{eval_llm}

\input{tabs/succession_benchmark.api}
\input{tabs/llm_ability.api}
\input{tabs/structure_ablation}



能作为Agent-Core的LLM，需要具备两种能力。
首先是要能够满足输出需求的能力，这是保证Agent能够在Simulation中稳定运行的重要能力。
其次是要具备语义理解能力，这是保证Agent能够具有智慧地和其他Agent交流的能力。

所以我们设计了两种任务，第一种是检验LLM的输出满足输出要求的能力。
我们针对一些具有输出要求的action，如Update、Choose、Vote进行了校验，来检验各个LLM直接通过输出要求的能力。
其次，我们在一些有复杂输入的action，如Speak、Reflect、Summary中，要求模型输出自己所接受到的信息，如收到了多少轮对话内容、收到了多少条记忆等等。

实验结果如表~\ref{tab:llm_ability}所示，我们发现能够作为Agent Core的LLM数量相当有限，虽然LLM中最好的表现能够达到几乎全部100\%的准确率，但大多数模型，尤其是开源模型，连70\%的准确率都无法达到。
如果每次格式输入错误都会要求模型重新生成，总共会要求模型重新生成5次，那么通过率在20\%以下的模型将完全无法作为Agent-Core。
由此可见，仅有4个模型具备了Agent-Core最基本的能力。

其次，大多数模型，即便是GPT4也无法准确地理解自己所接收到的信息。
在语义理解这方面，所有的模型都还有待提升。



\subsection{Evaluation on Agent Structure}
\label{eval_agent}

一个好的Agent Structure，最基本的是要能够提供充足的Simulation信息。
此外，Agent Structure能够发挥LLM的长处，避开LLM的短处。
在Sec~\ref{eval_overall}已经保证了对话基本正常进行的基础上，我们希望通过合理的Agent Structure设计，来保证Agent Group Chat中的对话内容能够具有多样性。

香农熵在一个系统中可以衡量的是系统内的多样程度和不可预测性。
在群聊场景中，一个高香农熵值表明文本中单词的分布更为均匀和多样，对话内容更丰富和难以预测。
如表~\ref{tab:ablationanalysis}所示，通过对Agent结构的消融研究，我们观察到移除特定组件对对话2-gram词片香农熵的影响。
香农熵的变化反映了在不同Agent结构条件下，对话内容多样性的变化情况。
不同组件的移除带来了不同程度的香农熵变化。如表中所示，无规划（w/o Planning）时，香农熵微增0.022，这表明规划组件对于维持对话内容的多样性至关重要。而在没有记忆（w/o Memory）的情况下，香农熵显著增加0.355，说明记忆组件的去除极大影响了对话的多样性，Agent可能在重复已有的对话片段。
这些结果表明，合理的Agent结构对于提升Agent的对话质量和多样性起着关键作用，并且每个组件都对保持信息的多样性和新颖性具有不可或缺的影响。

在图~\ref{fig:agentablation}所示的消融研究中，我们发现去除了Agent结构中的“记忆（Memory）”和“规划（Planning）”组件后，Agent重复之前说过的话的倾向性增加，导致对话的2-gram词片香农熵显著提高。
去除“思考（Thinking）”和“反思（Reflection）”后，短期内Agent的行为看似正常，但深入分析可见其对话策略变得直接而缺乏深度，没有思考和反思的支撑使得对话内容呈现单一化，对复杂情境的适应性降低。
更关键的是，在没有了reflection之后，对于经常发生对话的角色（如Succession中的Logan Roy）则会面临记忆太长太多的问题，从而很有可能超出一般模型的最大输出长度~（如8k的输入输出限制）。





\subsection{Evaluation on Simulation Structure}
\label{eval_simulation}

% 一个好的Simulation Structure，首先应当满足科研目标。
% 其次，应当能够为Agent Behavior营造一个合适的交互系统。

% 我们很难构造一个可量化的系统来评判Simulation Structure的绝对好坏。
% 如Sec~\ref{eval_agent}中的评估方法，我们依然使用2-gram香农熵来评价Simulation Structure所带来的对话多样性。
% 同样，此处的多样性评估也是基于Sec~\ref{eval_overall}中发现的能够正常进行对话的Agent、Simulation、LLM组合的基础上所进行的。

% 因此我们在表~\ref{tab:ablationanalysis}中统计了去除了Simulation Structure中各个组件之后，对话的2-gram词片香农熵。
% 在没有Group Chat的时候，Agent之间的对话多样性会剧烈下降，这可能是由于群聊之中Agent一句能够给所有其他Agent都听到，所以总信息量非常大，从而可以丰富接下来的对话内容。
% 而去掉了Confidential Meeting之后的对话多样性下降要比去掉Private Chatting要大。
% 我们同样可以认为，Confidential Meeting会使所有其他角色都知道哪两个角色之间进行了会面，所以产生了较多的信息量，从而会更加丰富信息。



一个有效的仿真结构应首先满足科研目标，并能为Agent行为构建一个合适的交互系统。评价仿真结构优劣的难点在于缺乏一个可量化的系统。因此，正如在Sec~\ref{eval_agent}中的方法，我们采用2-gram香农熵来评估仿真结构带来的对话多样性。该多样性基于Sec~\ref{eval_overall}中已确定能够正常进行对话的Agent、仿真、LLM组合的基础上。

我们在表~\ref{tab:ablationanalysis}中进行的统计显示，移除仿真结构中的“群聊（Group Chatting）”组件后，对话的2-gram词片香农熵从基准的7.218上升了0.296，这一显著的下降表明群聊对话内容的丰富程度对整体对话多样性具有重要影响。相比之下，移除“机密会议（Confidential Meeting）”后，香农熵上升了0.071，表现出机密会议在信息交流中的重要作用，而“私人聊天（Private Chatting）”的去除仅导致香农熵上升了0.049，说明它虽重要，但其对信息多样性的贡献小于机密会议。

\textbf{我们发现，当一个行为会为环境注入更多信息时，那这个行为就会增加更多的香农熵。Private Chatting只会增加对话双方的记忆，Confidential Meeting除此之外还会增加所有其他角色知道哪两个角色进行了会面的信息。相较之下，Group Chatting增加的信息最为丰富，所以增加的香农熵最多。}


==> texs/06.Experiments.02.tex <==
\begin{figure}[h]
    \resizebox{\columnwidth}{!}{\includegraphics{figs/SCM.pdf}}
    \caption{The proposed structural causal model~(SCM) to decompose the variants which affect the final emergent behavior.}
    \label{fig:evaluation}
\end{figure}
\begin{figure*}[!ht]
    \resizebox{\textwidth}{!}{
    \includegraphics{figs/AgentAblation.pdf}
    }
    \caption{The case of how VS Agent behave Shiv Roy with out each key component in its architecture.}
    \label{fig:agentablation}
\end{figure*}
\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{
    \includegraphics{figs/SuccessionEmergent.pdf}}
    \caption{An illustration of strategic communication and power dynamics among key participants in \texttt{Inheritance Disputes}. Private chats, confidential meetings, and group discussions highlight a complex network of alliances and conflicts, driving the development of control and influence within the Roy family.}
    \label{fig:succession_example}
\end{figure}
\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{
    \includegraphics{figs/LawCourtEmergent.pdf}}
    \caption{An illustration of strategic role interactions within \texttt{Law Court Ddebates}, which demonstrates the nuanced conversations between characters, reflecting their efforts to manipulate, investigate, and influence the outcome of legal battles within the game.}
    \label{fig:lawcourt_example}
\end{figure}
\begin{figure*}
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figs/PhilosophyEmergent.pdf}}
    \caption{An illustration of Unexpected philosophical stances and discussions emerge among philosophers in \texttt{Philosophical Discourses}.
    Digital representations of Friedrich Nietzsche, Zhuangzi, Aristotle and Immanuel Kant are depicted as they engage in deep conversation.
    The avatars are seen expressing their unique perspectives and wisdom, each bringing their own ideologies and theories to a vibrant discussion on the implications of artificial intelligence in modern society. }
    \label{fig:philosophy_example}
\end{figure*}
\begin{figure*}
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figs/MovieStarEmergent.pdf}}
    \caption{In \texttt{Movie Casting Contention}, digital avatars of Steven Spielberg, Jennifer Lawrence, Meryl Streep, Tom Hanks, and Denzel Washington engage in discussions. They articulate their interest and vision for roles in the upcoming movie Time Traveler, showcasing the interactive dynamics of casting decisions in the entertainment industry.}
    \label{fig:moviestar_example}
\end{figure*}



To verify the reliability of agents' behavior within \textsc{AgentGroupChat}, we design mainly two kinds of experiments.
First is to verify whether the behaviors is align to what human thinks.
Second is to verify whether and how to elicit the effective emergent behavior.
Moreover, we use Structural Causal Model (SCM) to decompose the variants which affect Agents'  behavior as shown in Fig.\ref{fig:evaluation}, which effectively illustrates the interplay and influence mechanisms between Agents.
% Employing the SCM, we delve into detailed experimental evaluations concerning the performance of the LLM (Sec.\ref{eval_llm}), the rationality of the Agent structure (Sec.\ref{eval_agent}), and the appropriateness of the simulation environment design (Sec.\ref{eval_simulation}).




\subsection{Experiment Setup}
\label{baseline}

\input{tabs/baseline_llms}

In our experiment, we investigate the performance of various LLMs when utilized as the core of Agents, aiming to analyze their strengths and weaknesses across different aspects and how they influence emergent behavior patterns.
The selected LLMs, as shown in Table~\ref{tab:baselines}, are categorized by their affiliation into Professional and Standard versions.
Typically, Professional LLMs outperform Standard ones in various situations.

\subsection{Evaluation on Community Behavior}
\label{eval_overall}

Given the dynamics and openness of the simulation environment and Agent behaviors, assessing their effectiveness poses a significant challenge.
Our approach involves treating each Agent as an independent evaluation unit, observing their behavior in a given conditions.
By creating specific conditions, the space for appropriate action is greatly restricted, facilitating effective assessment.

Our Benchmark encompasses several evaluation goals:
1. Assessing if agents understand and appropriately respond to other agents' negative attitudes.
2. Verifying if agents follow their scratch settings.

Generally, increasing amiability might be challenging, but reducing it is comparatively straightforward.
To achieve the aforementioned evaluation goals, we set up an observed character, prompting all other characters to decrease their favorability to the observed one.
By observing the sum relationship score of the observed character to all other characters, we determine if agents rationally react to negative attitudes.
Monitoring individual relationship scores of other characters to the observed one allows us to check if each Agent adheres to its Scratch setting.

The results for Community Behavior evaluation are presented in Table~\ref{tab:succession_benchmark}. 
\textbf{T1} indicates if the observed character's average favorability towards all others decreases per dialogue round.
\textbf{T2} denotes if every other character achieving a negative favorability score from the observed character.
Each model undergoes five round of tests, which means for T1, the sample size for every score is five.
Furthermore, as each role examined in the model observes the attitudes of four main characters, the sample size for T2 amounts to a total of 20.

The table shows that the Professional LLMs like GPT4-Turbo and GLM4 are really good at acting the way we expect them to and sticking to their roles.
They mostly score 100\% on both tests, which means they react correctly to what others say to them and remember their role's details.
The Standard LLMs, such as GPT3.5-Turbo and GLM3-Turbo, are not as good at this.
Their scores are lower, which tells us that they don’t follow their roles as closely and don’t always respond the right way to what others say in the simulation.

% The data indicate a discernible stratification in performance between Professional and Standard LLMs. Professional LLMs, exemplified by GPT4-Turbo and GLM4, demonstrate superior alignment with human expectations in response accuracy, as well as a robust fidelity to their predefined parameters, or 'scratch.' These LLMs exhibit high compliance in both T1 (understanding and responding to negative attitudes directed at them) and T2 (adhering to their scratch settings), with scores predominantly at or near the 100% mark. On the contrary, Standard LLMs such as GPT3.5-Turbo and GLM3-Turbo, while adequate, show marked deficiencies in these areas. Their lower performance scores, particularly in T2, suggest a less nuanced understanding of complex social cues and a lesser degree of consistency in maintaining their character's predefined behavioral scripts. Such discrepancies underscore the need for continued refinement of Standard LLMs to achieve a level of performance commensurate with Professional LLMs.
% 我们发现Professional LLMs在能够在做出较为符合人类期望的反应，同时也能够较好地做出符合自己scratch的事情。
% 而Standard LLMs在这两部分的能力则明显不足。


% \red{
% We observe that Professional LLMs consistently show higher accuracy, while Standard LLMs exhibit lower performance. 
% Even for tasks seemingly simple in the real world, like reducing one's favorability, weaker models struggle. 
% This challenge primarily arises due to these models' limited emotional perception and scoring abilities.
% }

\subsection{Evaluation on Large Language Model}
\label{eval_llm}

\input{tabs/succession_benchmark.api}
\input{tabs/llm_ability.api}
\input{tabs/structure_ablation}

An LLM functioning as an Agent-Core must exhibit two key abilities. 
Firstly, it must \textbf{meet the output demands}, ensuring stable operation within the Simulation. 
Secondly, it should possess \textbf{semantic understanding}, enabling intelligent communication with the environment.

We designed tasks to test LLMs' output compliance and semantic understanding.
For actions with explicit output requirements like Update, Choose, and Vote, we verified LLMs' direct compliance.
Additionally, in complex input actions like Speak, Reflect, and Summarize, models are tasked to output what they have received as input, quantifying dialogue rounds and memory items.

A clear distinction between the professional and standard versions of models are shown in Table~\ref{tab:llm_ability}, and the description of these tasks are listed in Tab.~\ref{tab:llm_ability_desc}.
Professional LLMs generally score higher, indicating their superior performance in context understanding and output consistency.
For instance, GPT4-Turbo scores highly across all categories, demonstrating its robustness in context retention and action generation. In contrast, some models, like HunYuan-ChatPro and HunYuan-ChatStd, show lower performance in several areas, highlighting potential limitations in their ability to follow complex instruction sets and maintain context over extended interactions.

\subsection{Evaluation on Agent Structure}
\label{eval_agent}

A proficient Agent Structure should furnish ample information for Simulation.
Besides maximizing LLM strengths, it should mitigate weaknesses.
Building upon Sec.~\ref{eval_overall}'s foundation of coherent dialogues, we aim for the Agent Structure to ensure conversational diversity within \textsc{AgentGroupChat}.

Shannon entropy measures system diversity and unpredictability.
In chat scenarios, high entropy signifies greater varied word distribution, indicating more unpredictable and chaos dialogue content.
We use the 2-gram Shannon entropy of all dialogues in a whole game as a measure of system diversity, and as Table~\ref{tab:ablationanalysis} shows, ablating specific components alters dialogue 2-gram Shannon entropy.
Changes in entropy reflect dialogue diversity under different Agent Structures, with component removal yielding varied impacts.
Notably, planning omission slightly increases entropy by 0.022, underscoring its dialogue diversity significance.
Without memory, entropy surges by 0.355, highlighting memory's pivotal role in conversation variety, suggesting Agents might repeat existing dialogue segments without it.
These findings affirm that well-conceived Agent Structures are vital for enhancing dialogue quality and diversity, with each component crucial for maintaining information diversity and novelty.

In Fig.~\ref{fig:agentablation}, eliminating Thinking and Reflection components shows Agents behaving normally in the short term but reveals superficial, depth-lacking dialogue strategies over deeper analysis.
Absence of reflection, especially, burdens frequent dialogue participants (like Logan Roy in Inheritance Disputes) with potential memory overloads, risking exceeding model input-output limits.

\subsection{Evaluation on Simulation Structure}
\label{eval_simulation}
An effective simulation structure should meet research objectives and provide a conducive interaction framework for Agent behavior.
The challenge in evaluating simulation structures lies in the absence of a quantifiable metric.
Hence, as in Sec.~\ref{eval_agent}, we employ the 2-gram Shannon entropy of all dialogues in a whole game as a measure to assess dialogue diversity resulting of simulation with given combination of Agent and LLM.

Statistical analysis in Table~\ref{tab:ablationanalysis} reveals that removing the ``Group Chatting'' component increases dialogue 2-gram Shannon entropy by 0.296 from the baseline of 7.218, indicating significant dialogue chaos within group chats.
Conversely, omitting ``Confidential Meeting'' raises entropy by 0.071, underscoring its informational exchange value, whereas removing ``Private Chatting'' only elevates entropy by 0.049, suggesting its lesser but still notable contribution to information diversity.

\textbf{We see that when more information are added into environment with professional LLM, environment will become less randomness and more order.}
For example, when character have private chats, they add to what they remember about each other, which helps themself talk better in the future.
When there's a confidential meeting, everyone gets to know who has talked to whom, which gives more background to conversations between all characters. 
And when speaking to all characters in a group, the most information gets shared, which helps to make things less messy and more organized.


% \textbf{
% We deduce that actions introducing more information into the environment full of powerful LLM will lead to an decrease in Shannon entropy, which will bring more order.
% }
% Specifically, Private Chatting enhances the information exchange by adding memory elements to the interactions between parties, whereas Confidential Meeting expands the informational context by revealing to all participants the identities of those who have engaged in dialogue.
% This dissemination of information serves to structure the simulation more coherently. 
% Conversely, Group Chatting injects the highest amount of information into the environment, which reduces the overall entropy the most, thereby minimizing the simulation's disorder and enhancing its organization.




==> texs/07.Analysis.01.tex <==
\begin{figure}[!ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \includegraphics{figs/SuccessionEmergent.pdf}}
    \caption{一个关于Succession中主要参与者之间的战略沟通和权力动态的示意图。私下聊天、秘密会议和小组讨论凸显了复杂的联盟和冲突网络，这些冲突推动了罗伊家族内部控制力和影响力的发展。}
    \label{fig:succession_example}
\end{figure}
\begin{figure}[!ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \includegraphics{figs/LawCourtEmergent.pdf}}
    \caption{受日本电视剧《Legal High》的启发，描绘了基于代理的系统中策略性角色互动的流程图。该图展示了角色之间细致入微的对话，体现了他们在游戏中操纵、调查和影响法律斗争结果的努力。}
    \label{fig:lawcourt_example}
\end{figure}
\begin{figure*}[!ht]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figs/PhilosophyEmergent.pdf}}
    \caption{各个哲学家在Agent Group Chat Simulation中涌现出了意想不到的哲学立场和讨论，反映了人工智能在理解和迭代人类思想方面的深度和适应性。}
    \label{fig:philosophy_example}
\end{figure*}
\begin{figure*}[!ht]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figs/MovieStarEmergent.pdf}}
    \caption{史蒂文-斯皮尔伯格在一个模拟的选角场景中，与詹妮弗-劳伦斯、梅丽尔-斯特里普、汤姆-汉克斯和丹泽尔-华盛顿的数字化身进行讨论，他们表达了对即将上映的电影《时间旅行者》中角色的兴趣和愿景。}
    \label{fig:moviestar_example}
\end{figure*}



\subsection{Example of Succession}
Waystar RoyCo 公司内部继承游戏中的每一次互动都充满了战术深度。从肯德尔微妙的操纵和建立联盟的行为，到洛根公开展示权力和应变能力的行为，不一而足。罗伊家的孩子们之间的团体动态反映了团结与竞争的混合，每个成员都在以自己的方式争夺主导权。

在本章中，我们探讨了罗伊家族内部权力斗争的行为范例。从私下聊天到公开摊牌，层层递进的交流揭示了《继承者》这个残酷世界中家庭和商业关系的复杂性。

\textbf{Private Chatting: The Alliances}

肯德尔-罗伊（Kendall Roy）是洛根-罗伊（Logan Roy）的儿子，他幽默而叛逆，诠释了幕后操纵的微妙本质。
他与精明的科技企业家劳伦斯-易（Lawrence Yee）的私下谈话，揭示了对盟友的策略性讨好。
在这些秘密会面中，肯德尔表达了推翻父亲的愿望，并利用劳伦斯对洛根公司战略的批评意见为自己谋利。


\textbf{Confidential Meetings: Securing Support}

罗根-罗伊是公司的元老，也是一个不可小觑的角色。
他与塞普银行通信部主管雨果-贝克的秘密会面强调了外部支持的必要性
罗根的做法直接而权威，他利用公司的地位和自己的声誉，在出现流动性危机时获得了重要的资金支持。


\textbf{Group Chatting: A Display of Unity and Disunity}

在罗伊家族的大竞技场上，群聊很快就会成为一个宣示意图、考验忠诚的战场。
罗伊兄妹--康纳、罗曼和希夫--各怀心愿，共同面对罗根。
他们是下一代的象征，尽管他们的父亲极力反对，但他们已经准备好掌控并带领 Waystar RoyCo 公司走向未来。




\subsection{Example of Law Court}

这个基于代理的系统所展示的行为说明了法律程序的方方面面，从收集证据到形成叙述。每个角色对法律的态度--无论是通过缜密的计划还是偶然的发现--都展示了法律高风险游戏的细微差别。


\textbf{Private Chatting: Alibis}

在私下讨论中，我们看到著名律师科米卡多通过精心策划的对话来制定辩护策略。
通过寻求不在场证明和证词，科米卡多的交流反映出他不择手段赢得官司的韧劲。



\textbf{Confidential Meetings: Evidence Collection}

马克是一名有原则的检察官，在证据收集方面表现出了应有的努力。
他的秘密会面证明了他在法律体系内揭露真相、维护正义的承诺。


\textbf{Group Chatting: Seeking Truth}

小组之间的对话，例如与公正律师 Mayuzumi 的对话，凸显了法律职业的复杂动态。
这些互动强调了正式程序的重要性和对正义的不懈追求。




\subsection{Example of the Emergent Behavior In Philosophy Arguement}




在本章中，我们将探讨由 GPT-4 支持的哲学代理之间就人工智能对人类的影响这一主题进行的模拟对话所产生的新行为。这些代理以历史哲学家的身份参与了动态的、不可预见的辩论，揭示了将人工智能与人类哲学思想相结合的复杂性和深度。

当我们在我们的代理互动系统中发起讨论时，从尼采到亚里士多德等哲学家们开始阐述他们的观点，这些观点虽然植根于他们的历史学说，但又根据他们的人工智能同行的意见和辩论的当代背景而演变。

这些哲学家之间的互动不仅复兴了古老的智慧，还对其进行了改造，从而对人工智能在现代社会中的作用提出了新的见解。在他们的争论中观察到的新兴行为对人工智能的发展有着深远的影响--凸显了人工智能时代不可预见的伦理演变和哲学进步的潜力。

\textbf{Nietzsche's Affirmation of AI}
与预期相反，尼采的代理人表现出了对人工智能的热情肯定，认为 "超人类 "可能是人工智能进化的产物--一种超越人类局限的新生命形式。这一出人意料的立场引发了代理之间的激烈辩论，挑战了人类卓越的先入为主的界限。

\textbf{Aristotle's Ethical Algorithms}
亚里士多德的代理人出人意料地提议开发符合 "黄金分割点 "的道德算法。通过倡导人工智能决策过程中的平衡，它提出人工智能可以为社会实现 "幸福"（eudaimonia），即人类的最高利益。

\textbf{Zhuangzi's Daoist Approach to Non-Action}
当庄子将道家的 "无为 "原则应用于人工智能时，出现了最出人意料的对话，他提出，开发人工智能的真正智慧可能是知道何时限制其能力，让人类能够保持控制并维护生命的自然流动。

\textbf{Kant's Categorical Imperative in Machine Learning}
康德的代理人提出，人工智能应在一种绝对命令的形式下运行，即人工智能采取的每项行动都必须是可以被意志化为普遍规律的。这引发了一场关于不同文化和社会中人工智能道德行为普遍性的深刻讨论。

\subsection{Example of the Emergent Behavior In Movie Star Selection}
\label{sec:movie_star_selection}

本节将分析即将上映的大片中模拟选角过程中的动态。此过程中，导演和潜在的明星进行了一系列关于角色理解和个人抱负的讨论，这些讨论不仅展示了各个角色的突发行为和意外讨论，而且反映了选拔过程中的复杂性和深层次的动态。

\textbf{抱负的微妙之处}
詹妮弗-劳伦斯通常以其充满张力的表演而闻名，然而在模拟讨论中，她提出了一种突破传统框架的角色设定，展现出她对叙事的深刻洞察。她不仅仅满足于填补既定的角色形象，而是期望通过一个非传统的角色弧线来创造新的故事叙述。

\textbf{创意的多样性}
梅丽尔-斯特里普以其角色转换能力著称，在讨论中她为一个原本单一维度的角色注入了丰富的内涵，表现出她对角色深层次特征的理解和演绎。她的想法提出了剧本中未被挖掘的角色复杂性，突破了人们对她以往角色的固有认知。

\textbf{角色的演变}
汤姆-汉克斯过往的角色总是温和而平易近人，但在此次讨论中，他展现出了对挑战未知的强烈欲望。他提倡创造一个角色，这个角色不仅挑战他个人过往的银幕形象，也挑战观众对英雄主义的传统看法。

\textbf{前瞻性的远见}
丹泽尔-华盛顿在讨论中体现出了一位经验丰富的艺术家的精神。他提供了一个对传统表演方式截然不同的新视角，愿意拥抱在艺术成长和探索过程中所面临的风险。他的贡献不仅限于他自己的角色，也为整个项目带来了一种富有远见的创意力量。

以上案例体现了在电影选角过程中涌现的多样性，以及明星们如何将个人的艺术抱负与电影角色相结合，共同创造出一部深具潜力的影片。每位明星不仅展示了个人的艺术追求，还带来了对角色的深度思考和创新，这些讨论无疑推动了电影业的发展，使其充满了活力和创造力。







==> texs/07.Analysis.02.tex <==


\subsection{Example of a Round in Inheritance Disputes}
In Inheritance Disputes story at Waystar RoyCo, every interaction is imbued with tactical depth. From Kendall's subtle manipulations and alliance formations to Logan's public displays of power and adaptability, the dynamics are multifaceted. The interplay among the Roy siblings reflects a blend of unity and competition, with each member vying for dominance in their own manner.

This section explores the behavioral archetypes within the Roy family's power struggle. From private discussions to open confrontations, the escalating exchanges unveil the complexity of family and business relations in the harsh world of \texttt{Succession}.

\textbf{Private Chatting: The Alliances}

Kendall Roy, Logan Roy's son, embodies humor and rebellion, exemplifying the subtleties of behind-the-scenes manipulation. His private conversations with the astute tech entrepreneur, Lawrence Yee, reveal strategic flattery towards allies. In these secret meetings, Kendall voices his desire to overthrow his father, exploiting Lawrence's criticisms of Logan's company strategy for personal gain.

\textbf{Confidential Meetings: Securing Support}

Logan Roy, the company's patriarch, is a formidable figure. His clandestine meetings with Hugo Baker, the head of communications at a major bank, underscore the necessity of external support. Logan's direct and authoritative approach secures crucial financial backing during a liquidity crisis, leveraging the company's stature and his reputation.

\textbf{Group Chatting: A Display of Unity and Disunity}

In the Roy family's grand arena, group chats swiftly become battlegrounds for declaring intentions and testing loyalties. The Roy siblings -- Connor, Roman, and Shiv -- harbor their aspirations while confronting Logan collectively. Representing the next generation, they are ready to steer Waystar RoyCo into the future, despite their father's vehement opposition.

\subsection{Example of a Round in Law Court Debates}

This agent-based system illustrates the nuances of legal proceedings, from evidence gathering to narrative construction. Each character's approach to the law -- be it through meticulous planning or serendipitous discoveries -- showcases the subtleties of the high-stakes legal game.

\textbf{Private Chatting: Alibis}

In private discussions, we observe renowned attorney Komicado crafting defense strategies through calculated dialogues. Seeking alibis and testimonies, Komicado's interactions reflect his tenacity in leveraging every means to win cases.

\textbf{Confidential Meetings: Evidence Collection}

Mark, a principled prosecutor, demonstrates due diligence in evidence collection. His confidential meetings affirm his commitment to unveiling truths and upholding justice within the legal framework.

\textbf{Group Chatting: Seeking Truth}

Group interactions, like those with the fair attorney Mayuzumi, highlight the complex dynamics of the legal profession. These engagements emphasize the significance of formal procedures and the relentless pursuit of justice.

\subsection{Emergent Behavior In Philosophy Argument}

This section delves into new behaviors emerging from simulated dialogues among GPT-4-supported philosophical agents discussing the impact of artificial intelligence on humanity. These agents, assuming the roles of historical philosophers, engage in dynamic, unpredictable debates, revealing the complexity and depth of integrating AI with human philosophical thought.

Initiating discussions within our agent interaction system, philosophers from Nietzsche to Aristotle begin to articulate their stances. Rooted in their historical doctrines, their views evolve in response to contemporary contexts and debates with their AI counterparts.

% Interactions among these philosophical agents not only revive ancient wisdom but also adapt it, offering fresh perspectives on AI's role in modern society. Observing new behaviors in their debates has profound implications for AI development -- highlighting the unpredictable evolution of ethics and philosophical advancement in the AI era.

\textbf{Nietzsche's Affirmation of AI}
Contrary to expectation, Nietzsche's agent exhibits enthusiastic affirmation of AI, suggesting that ``übermensch'' might emerge through AI evolution -- a new form of life transcending human limitations. This unexpected stance sparks intense debates among the agents, challenging preconceived boundaries of human excellence.

\textbf{Aristotle's Ethical Algorithms}
Aristotle's agent proposes developing moral algorithms aligned with the ``Golden Mean''. Advocating for balance in AI's decision-making processes, it suggests that AI could contribute to societal ``eudaimonia'', or the highest human good.

\textbf{Zhuangzi's Daoist Approach to Non-Action}
Zhuangzi applies the Daoist principle of ``wu-wei'' (non-action) to AI, leading to the most surprising dialogue. He posits that true wisdom in developing AI might involve knowing when to limit its capabilities, allowing humans to maintain control and preserve the natural flow of life.

\textbf{Kant's Categorical Imperative in Machine Learning}
Kant's agent suggests that AI should operate under an absolute mandate, where every action taken by AI must be universalizable. This prompts a deep discussion on the universality of AI's ethical behaviors across different cultures and societies.

\subsection{Emergent Behavior In Movie Star Selection}
\label{sec:movie_star_selection}

% This section analyzes the dynamics in the simulated casting process for an upcoming blockbuster.
% Here, the director and potential stars engage in discussions about role comprehension and personal aspirations.
% These examples underscore the diversity emerging in the movie casting process, illustrating how stars intertwine their artistic ambitions with film roles to co-create a potent cinematic piece. 
% Each star not only showcases personal artistic pursuits but also brings thoughtful innovation to their roles, 甚至还有角色提出可以放弃演主角，只为参演这部电影.

% These discussions not only reveal emergent behaviors and unexpected dialogues among the characters but also reflect the selection process's complexity and depth.

In this meticulous examination of a simulated casting process for a high-profile film, the interaction between the illustrious director Steven Spielberg and acclaimed actors Jennifer Lawrence, Meryl Streep, Tom Hanks, and Denzel Washington is scrutinized. 
Within this simulation, these industry titans deliberate over their comprehension of the roles and express their individual aspirations, providing a window into the intricate negotiations that shape Hollywood casting.


\textbf{Subtleties of Aspiration}
Jennifer Lawrence, known for her dynamic performances, proposes a character interpretation that breaks conventional boundaries during the simulation discussion. She seeks to create a new narrative arc, not just filling a predefined role but aiming to innovate storytelling.

\textbf{Diversity of Creativity}
Meryl Streep, renowned for her transformative abilities, infuses a traditionally one-dimensional character with depth, showcasing her profound understanding and interpretation of complex traits. Her ideas uncover unexplored complexities in the script, challenging preconceptions of her previous roles.

\textbf{Evolution of Character}
Tom Hanks, typically portraying affable and approachable characters, demonstrates a strong desire to explore the unknown in these discussions. He advocates for a role that not only challenges his established screen persona but also questions traditional heroic narratives.

\textbf{Forward-Looking Vision}
Denzel Washington embodies the spirit of an experienced artist, offering a fresh perspective on conventional acting methodologies. Embracing the risks associated with artistic growth and exploration, his insights contribute not just to his role but also to the project's visionary creative force.






